Temporal Logic Control for Nonlinear Stochastic Systems Under Unknown Disturbances

In this paper, we present a novel framework to synthesize robust strategies for discrete-time nonlinear systems with random disturbances that are unknown, against temporal logic specifications. The proposed framework is data-driven and abstraction-based: leveraging observations of the system, our approach learns a high-confidence abstraction of the system in the form of an uncertain Markov decision process (UMDP). The uncertainty in the resulting UMDP is used to formally account for both the error in abstracting the system and for the uncertainty coming from the data. Critically, we show that for any given state-action pair in the resulting UMDP, the uncertainty in the transition probabilities can be represented as a convex polytope obtained by a two-layer state discretization and concentration inequalities. This allows us to obtain tighter uncertainty estimates compared to existing approaches, and guarantees efficiency, as we tailor a synthesis algorithm exploiting the structure of this UMDP. We empirically validate our approach on several case studies, showing substantially improved performance compared to the state-of-the-art.

==> Sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

The synthesis of safe strategies for stochastic systems is critical in ensuring \emph{reliable} and \emph{safe} operations in domains such as robotics, autonomous vehicles, and cyber-physical systems \citep{belta2005discrete,lavaei2022automated}. A key challenge arises when the system dynamics include \emph{unknown} random disturbances, making it difficult to account for uncertainties while guaranteeing performance against high-level complex specifications. Existing methods often assume known distributions for the disturbances or rely on abstractions with overly conservative uncertainty estimates, limiting their scalability and applicability to complex systems. This paper aims to address these gaps by presenting a novel framework to synthesize optimal strategies for nonlinear stochastic systems with unknown disturbances, ensuring both formal guarantees and computational efficiency.  

% Our framework employs a data-driven, abstraction-based approach. From a set of system observations, we construct a high-confidence abstraction in the form of an uncertain Markov decision process (UMDP), a flexible model capable of handling complex uncertainty. Unlike existing techniques, which often rely on interval-based abstractions or conservative statistical assumptions, our framework uses convex polytopes to represent the uncertainty in transition probabilities between states by using a 2-layered discretization--fine and coarse. We use two concentration inequalities to learn these bounds as well as the support of the unknown distribution. Incportating them in the UMDP leads to tighter uncertainty sets, yielding less conservative probabilistic guarantees. Exploiting this UMDP structure, we introduce an algorithm that ensures strategy synthesis on the resulting UMDP is computationally efficient, reducing to simpler than linear programming problems used on standard UMDPs. By incorporating the uncertainty stemming from both abstraction errors and data limitations, our framework provides robust strategies even under limited or noisy observations. 

Our framework employs a data-driven, abstraction-based approach to strategy synthesis for stochastic systems with unknown noise under \textit{linear temporal logic over finite traces} (\LTLf) \citep{de2013linear} specifications. Starting with data from the system's trajectories, we construct a high-confidence abstraction in the form of an uncertain Markov decision process (UMDP) \citep{iyengar2005robust}, a flexible model that captures complex uncertainties. Unlike existing methods relying on interval-based abstractions or conservative assumptions, our framework represents transition probability uncertainties as convex polytopes. These sets are derived through a novel two-layer discretization scheme and learning the support of the unknown disturbance. This leads to tighter uncertainty sets and less conservative results compared to existing methods. Exploiting this UMDP structure, we introduce a synthesis algorithm for \LTLf specifications that simplifies the computation, reducing the complexity of standard UMDP linear programming approaches. By incorporating uncertainties from both abstraction errors and data limitations, our framework yields a strategy that is robust. Our empirical evaluations over various types of systems reveals the efficacy of this approach over existing methods, namely in data efficiency, tightness of results, and scalability.

The main contributions of this paper are fourfold: (i) a novel framework for synthesizing strategies for nonlinear stochastic systems under non-additive, unknown disturbances with \LTLf specifications, (ii) a distribution-agnostic, data-driven construction of UMDP abstraction with a specific structure that reduces conservatism of existing abstraction-based techniques, (iii) an efficient tailored synthesis algorithm for this UMDP abstraction, which does not introduce additional conservatism %results in tight error bounds
, and (iv) a series of case studies and benchmarks that show superiority of the framework over the state-of-the-art, with up to $3$ orders of magnitude improvement in sample complexity and an order of magnitude reduction in computation time.
% the framework's superiority over the state-of-the-art, achieving up to $3$ orders of magnitude improvement in sample complexity and an order of magnitude reduction in computation time.


\paragraph{Related Work}

% Over the past decade, interval Markov decision processes (IMDPs) \citep{lahijanian2015formal,givan2000bounded} have become a successful abstraction for stochastic systems. By allowing transition probabilities to be uncertain and confined to intervals, IMDPs are able to capture the full range of behaviors in the original system. For instance, \citep{cauchi2019efficiency} introduces an efficient approach for abstracting linear systems with additive Gaussian noise to IMDPs, while \citep{skovbekk2023formal} extends this abstraction to a broader class of dynamics, including those nonlinear in state and disturbance, by partitioning the disturbance space.

% Uncertain MDPs (UMDPs) \citep{iyengar2005robust,el2005robust} generalize IMDPs by allowing transition probability distributions to belong to more complex sets, extending beyond simple intervals. \citep{wolff2012robust} explores strategy synthesis in UMDPs against linear temporal logic specifications, and \citep{gracia2025efficient} presents an efficient algorithm for strategy synthesis in UMDPs, particularly for reach-avoid specifications.

% Interval Markov decision processes (IMDPs) \citep{lahijanian2015formal,givan2000bounded} have become a successful abstraction for stochastic systems by representing uncertain transition probabilities within intervals, capturing the full range of system behaviors. For example, \citep{cauchi2019efficiency} efficiently abstracts linear systems with additive Gaussian noise, and \citep{skovbekk2023formal} extends this to more complex dynamics, including nonlinear systems. Uncertain MDPs (UMDPs) \citep{iyengar2005robust,el2005robust} generalize IMDPs by allowing transition probabilities to belong to more complex sets, and have been used in strategy synthesis against rich specifications such as linear temporal logic (LTL) \citep{wolff2012robust}. In many practical scenarios, however, system models are unavailable and must be estimated from data. 

% To address model uncertainty, some works have proposed leveraging Gaussian processes regression \citep{jackson2021strategy}, neural networks \citep{adams2022formal}, and ambiguity sets \citep{gracia2022distributionally}, which are then abstracted as IMDPs or UMDPs. Other works utilize statistical tools, such as the scenario approach, to learn abstractions for stochastic \citep{badings2023robust,badings2023probabilities}, non-deterministic \citep{kazemi2024data}, and deterministic systems \citep{coppola2022data,coppola2023data}. 
% Some works, such as \citep{lechner2022stability,badings2024learning,mazouz2024piecewise}, leverage knowledge of disturbance distributions to deal with stochastic systems with general dynamics through super-martingales and barrier functions.  All these works assume known disturbance. 

% When disturbance distributions are uncertain, existing methods combine IMDP abstractions with statistical tools like the scenario approach \citep{badings2023robust,badings2023probabilities,schon2023bayesian}. 
% For certifying safety in systems with unknown noise distributions, barrier functions are employed \citep{mathiesen2023inner}.
% % , and barrier certificates are also used in \citep{salamati2021data} for safety verification of systems with unknown dynamics and disturbance distributions, albeit under certain assumptions. 
% Another line of research focuses on constructing a Wasserstein ambiguity set from data samples, which can confidently contain the unknown probability distribution, and then abstracting the system as a UMDP \citep{gracia2022distributionally}.
% All these works however assume either simple dynamics or additive noise.

% % Another line of research focuses on constructing a Wasserstein ambiguity set from data samples, which can confidently contain the unknown probability distribution, and then abstracting the system as a UMDP \citep{gracia2024data}.

% % However, much of the existing literature typically assumes simpler system models, such as linear dynamics or additive noise \citep{cauchi2019efficiency,schon2023bayesian,badings2023robust,badings2023probabilities}, or presumes that disturbance distributions are known. 

% For general dynamics with unknown disturbance distribution, to the best of our knowledge, only two works exist \citep{salamati2021data,gracia2024data}.  Specifically, \citep{salamati2021data} provides safety verification using barrier certificates, and \citep{gracia2024data} extends the ambiguity set approach in \citep{gracia2022distributionally} for control synthesis for LTL specifications.  Both works, however, assume that certain distribution-related quantities—such as variance or support—are known, which is unrealistic in many cases. Moreover, both approaches suffer from high sample complexity, particularly when high confidence levels are required.  Our work addresses both of these shortcomings; we make no assumption about disturbance distribution, and our approach is data efficient and scalable.

% To the best of our knowledge, only \citep{salamati2021data} and our previous work \citep{gracia2024data} address systems with general dynamics without assuming a known disturbance distribution. Both works, however, assume that certain distribution-related quantities—such as variance or support—are known, which is unrealistic in many cases. Moreover, both approaches suffer from high sample complexity, particularly when high confidence levels are required.


% A class of abstractions of stochastic systems that has proved success in the past decade are interval Markov decision processes (IMDPs) \citep{lahijanian2015formal,givan2000bounded}. By letting the transition probabilities be uncertain and lie within intervals, these abstractions are able to capture all behaviors of the original system. For example, \citep{cauchi2019efficiency} proposes an efficient approach to abstract linear systems with additive Gaussian noise to IMDPs. \citep{skovbekk2023formal} obtains IMDP abstractions for a broader class of dynamics, namely, those nonlinear in state and disturbance, by partitioning the space of the disturbance.

% Uncertain MDPs (UMDPS) \citep{iyengar2005robust,el2005robust} are a generalization of IMDPs, in which the transition probability distributions belong to more complex sets than those defined by intervals in the transition probabilities.
% \citep{wolff2012robust} considers the setting of strategy synthesis in UMDPs against linear temporal logic specifications. In \citep{gracia2025efficient}, the authors provide an efficient algorithm for strategy synthesis on a more general class of UMDPs against reach-avoid specifications. 

% However, in many practical scenarios, a system model is not available and needs to be estimated from data. To this end and to cope with model uncertainty, some works have proposed to leverage Gaussian processes \citep{jackson2021strategy}, neural networks \citep{adams2022formal} and ambiguity sets \citep{gracia2022distributionally}, and then abstracting the learned model as an IMDP or UMDP. Others leverage statistical tools such as the scenario approach to learn an abstraction of stochastic \citep{badings2023robust,badings2023probabilities}, non-deterministic \citep{kazemi2024data}, and deterministic systems \citep{coppola2022data,coppola2023data}. In particular, when the distribution of the disturbances is uncertain, existing works propose to use IMDP abstractions in tandem with statistical tools such as the scenario approach \citep{badings2023robust,badings2023probabilities}. Other works choose to certify safety for systems with unknown noise distributions using barrier functions \citep{mathiesen2023inner}. Barrier certificates are also employed in \citep{salamati2021data} for safety verification of systems of unknown dynamics and unknown disturbance distribution, but under appropriate assumptions on these. 

% Another line of work proposes to use the data samples to construct a Wasserstein ambiguity set, which is guaranteed to contain the unknown probability distribution with high confidence,  and abstract the system to a UMDP \citep{gracia2024data,gracia2025efficient}.

% Leveraging knowledge of the disturbance's distribution, \citep{lechner2022stability,badings2024learning} and \citep{mazouz2024piecewise} deal with stochastic systems with general dynamics via super-martingales and barrier functions, respectively.

% However, existing literature usually considers either relatively simple system models, e.g., linear dynamics and/or additive noise \citep{cauchi2019efficiency,schon2023bayesian,badings2023robust,badings2023probabilities}, or assume that the distribution of the disturbance is known. To the best of our knowledge, the only works that are suited for systems with general dynamics and without assuming a known distribution for the noise are \citep{salamati2021data} and our previous work \citep{gracia2024data}. However, both works assume that some quantities related to the distribution of the disturbances, such as variance or support, are known, which is unrealistic in some cases. Additionally, the sample complexity of both approaches is high, especially when high confidences are needed.


% When the system model is unknown and has to be estimated from data, 




\iffalse
    Interval Markov decision processes (IMDPs) \citep{lahijanian2015formal,givan2000bounded} have become a successful abstraction for stochastic systems by representing uncertain transition probabilities within intervals, capturing the full range of system behaviors. For example, \citep{cauchi2019efficiency} efficiently abstracts linear systems with additive Gaussian noise, and \citep{skovbekk2023formal} extends this to more complex dynamics, including nonlinear systems. Uncertain MDPs (UMDPs) \citep{iyengar2005robust,el2005robust} generalize IMDPs by allowing transition probabilities to belong to more complex sets, and have been used in strategy synthesis against rich specifications such as linear temporal logic (LTL) \citep{wolff2012robust}. In many practical scenarios, however, system models are unavailable and must be estimated from data. 
    
    To address model uncertainty, some works have proposed leveraging Gaussian processes regression \citep{jackson2021strategy}, neural networks \citep{adams2022formal}, and ambiguity sets \citep{gracia2022distributionally}, which are then abstracted as IMDPs or UMDPs. Other works utilize statistical tools, such as the scenario approach, to learn abstractions for stochastic \citep{badings2023robust,badings2023probabilities}, non-deterministic \citep{kazemi2024data}, and deterministic systems \citep{coppola2022data,coppola2023data}. 
    Some works, such as \citep{lechner2022stability,badings2024learning,mazouz2024piecewise}, leverage knowledge of disturbance distributions to deal with stochastic systems with general dynamics through super-martingales and barrier functions.  All these works assume known disturbance. 
    
    When disturbance distributions are uncertain, existing methods combine IMDP abstractions with statistical tools like the scenario approach \citep{badings2023robust,badings2023probabilities,schon2023bayesian}. 
    For certifying safety in systems with unknown noise distributions, barrier functions are employed \citep{mathiesen2023inner}.
    % , and barrier certificates are also used in \citep{salamati2021data} for safety verification of systems with unknown dynamics and disturbance distributions, albeit under certain assumptions. 
    Another line of research focuses on constructing a Wasserstein ambiguity set from data samples, which can confidently contain the unknown probability distribution, and then abstracting the system as a UMDP \citep{gracia2022distributionally}.
    All these works however assume either simple dynamics or additive noise.
    
    % Another line of research focuses on constructing a Wasserstein ambiguity set from data samples, which can confidently contain the unknown probability distribution, and then abstracting the system as a UMDP \citep{gracia2024data}.
    
    % However, much of the existing literature typically assumes simpler system models, such as linear dynamics or additive noise \citep{cauchi2019efficiency,schon2023bayesian,badings2023robust,badings2023probabilities}, or presumes that disturbance distributions are known. 
    
    For general dynamics with unknown disturbance distribution, to the best of our knowledge, only two works exist \citep{salamati2021data,gracia2024data}.  Specifically, \citep{salamati2021data} provides safety verification using barrier certificates, and \citep{gracia2024data} extends the ambiguity set approach in \citep{gracia2022distributionally} for control synthesis for LTL specifications.  Both works, however, assume that certain distribution-related quantities—such as variance or support—are known, which is unrealistic in many cases. Moreover, both approaches suffer from high sample complexity, particularly when high confidence levels are required.  Our work addresses both of these shortcomings; we make no assumption about disturbance distribution, and our approach is data efficient and scalable.
\fi
Abstractions of stochastic systems to finite Markov decision processes (MDPs) are powerful tools for controller synthesis on highly-complex systems under complex logic specifications \citep{lavaei2022automated}. In particular, 
Interval MDPs (IMDPs) \citep{lahijanian2015formal,givan2000bounded} abstract systems by presenting uncertain transition probabilities within intervals, capturing the full range of system behaviors. For example, \citep{cauchi2019efficiency} efficiently abstracts linear systems with additive Gaussian noise, while \citep{skovbekk2023formal} extends this to nonlinear dynamics. Uncertain MDPs (UMDPs) \citep{iyengar2005robust,el2005robust} generalize IMDPs by allowing transition probabilities to belong to more complex sets and have been used for strategy synthesis against specifications such as linear temporal logic (LTL) \citep{wolff2012robust}. However, these abstractions typically require system models, which are often unavailable in practice.
% and must be learned from data.

To address model uncertainty, existing methods leverage Gaussian processes \citep{jackson2021strategy}, neural networks \citep{adams2022formal}, and ambiguity sets \citep{gracia2022distributionally}, which are then abstracted as IMDPs or UMDPs. Statistical tools like the scenario approach are also used to abstract stochastic \citep{badings2023robust,badings2023probabilities}, non-deterministic \citep{kazemi2024data}, and deterministic systems \citep{coppola2022data,coppola2023data}. Also, techniques like super-martingales and barrier functions enable safety verification and control for general dynamics \citep{lechner2022stability,badings2024learning,mazouz2024piecewise}, by assuming, however, that the disturbance distribution is known.

When disturbance distributions are uncertain, some works combine IMDP abstractions with statistical tools %like the scenario approach 
\citep{badings2023robust,badings2023probabilities,schon2023bayesian}, while others employ barrier certificates with the scenario approach for safety verification \citep{mathiesen2023inner}. Others  \citep{gracia2025efficient} construct Wasserstein ambiguity sets from data samples to abstract systems as UMDPs, which account for the uncertainty regarding the unknown distributions. However, these methods typically assume simple dynamics or additive noise. 
For general dynamics with unknown disturbance distributions, only a few works exist. \citep{salamati2021data} uses barrier certificates for safety verification, and \citep{gracia2024data} extends the ambiguity set approach to nonlinear dynamics, formally characterizing the guarantees of these approaches. Both assume that certain distribution-related properties, such as variance or support, are known—an assumption often unrealistic in practice, and also suffer from high sample complexity, especially under high-confidence requirements.  
Our work overcomes these limitations by removing assumptions about disturbance distributions and offering a data-efficient and scalable approach suitable for systems with general dynamics.

==> Sections/2_problem_formulation.tex <==
\section{Problem Formulation}

In this work the focus is on discrete-time stochastic systems given by
%
\vspace{-2mm}
\begin{align}
\label{eq:sys}
    \x_{k+1} = f(\x_k,u_k,\w_k),
\end{align}
%
where $\x_k\in\reals^n$ denotes the state at time $k\in\naturals_0$, $u_k\in U  \subset \reals^m$ is the control input chosen from a finite set $U$, and $\w_k\in W \subseteq \reals^d$ is the disturbance. The latter is a sequence of independent and identically distributed (i.i.d.) random variables on the probability space $(W,\mathcal{B}(W), P_W)$, with $\mathcal{B}$ being the Borel $\sigma$-algebra on $W$, being the support $W$ and probability distribution $P_W$ of $\w_k$ \emph{unknown}. The (possibly nonlinear) vector field $f:\reals^n\times U\times W \rightarrow \reals^n$ is assumed to be Lipschitz continuous on its third argument, uniformly for all values of its first argument on some set. 

\vspace{-2mm}
\begin{assumption}
\label{ass:lipschitz}
    There exists a set $X\subset\reals^n$, such that, for every $u\in U$, there exists a constant $L_u >0$ 
    such that, for all $x\in X$, $w,w'\in W$, it holds that $\|f(x, u, w) - f(x, u, w')\| \le L_u \|w - w'\|$.
\end{assumption}
% 
\vspace{-2mm}
In lieu of unknown $W$ and $P_W$, we assume a dataset on the disturbance is available.
\vspace{-2mm}
\begin{assumption}
\label{ass:samples}
    A set $\{\boldsymbol{\hat w}^{(i)}\}_{i=1}^N$ of $N$ i.i.d. samples from $P_W$ is available.
\end{assumption}
%
% \begin{remark}
    % Although Assumption~\ref{ass:samples} may seem strong since, in general, only observations of the state and control can be collected, in many practical cases we are able to obtain samples from $P_W$ from state-control observations. Let $S_x=\{(\hat x^{(i)}, \hat u^{(i)}, \boldsymbol{\hat y}^{(i)})\}_{i=1}^N$, where $\boldsymbol{\hat y}^{(i)}=f(\hat x^{(i)}, \hat u^{(i)}, \boldsymbol{\hat w}^{(i)})$ for some $\boldsymbol{\hat w}^{(i)}$ sampled from $P_w$ randomly. Then, if $f$ is linear in $w$ or, more generally, if $S_x$ is obtained where $f(\hat x^{(i)}, \hat u^{(i)},\cdot):W\longrightarrow\mathbb{R}^n$ is injective, we can invert $f$ to solve for the samples $\boldsymbol{\hat w}^{(i)}$. Note that global injectivity of $f$ is not needed and, since $f$ is known and the obtained samples $\boldsymbol{\hat w}^{(i)}$ do not depend on $\hat x^{(i)}, \hat u^{(i)}$, obtaining samples on a small region of the space $X\times U$ is enough to characterize $P_W$, and thus, the system's behavior on the entire space $X\times U$. Such regions of injectivity exist in most systems of practical interest, for example, in all the case studies we consider in Section~\ref{sec:case_studies}.
% \end{remark}
Assumption~\ref{ass:samples} is commonly made in related work \citep{badings2023robust,gracia2024data} and can be practically satisfied through, e.g., observations of the state and control. This is evident when $f$ is affine in $\w_k$; otherwise, it suffices for $f$ to be injective over only a subset of $\mathbb{R}^n$ as discussed in \citep{gracia2024data}. This condition is met by many practical systems, like those in our case studies.

% For instance, $f$ is injective Such regions of injectivity exist in most systems of practical interest, for example, in all the case studies we consider in Section~\ref{sec:case_studies}.

Given $x_0,\ldots,x_K \in \mathbb{R}^n$, $u_0,\dots,u_{K-1}\in U$, and $K \ge 0$, we denote a finite \emph{trajectory} of System~\eqref{eq:sys} by $\pathX =x_0 \xrightarrow{u_0}% x_1 \xrightarrow{u_1}  
\ldots \xrightarrow{u_{K-1}} x_K$. We let $|\pathX|$ denote the length of $\pathX$, define $\PathX$ as the set of all trajectories with $|\pathX|<\infty$ and denote by $\pathX(k)$ 
the state of $\pathX$ at time $k\in\{0,\dots, |\pathX|\}$. 
%\ig{To be consistent with our definition of path of the robust MDP, should we enforce that $x_{k+1}$ must be in the reachable set of $x_k,u_k,W$?}
%\ML{good quesiton. I think it's not needed bc once probability measure over paths is defined, then the probability of the paths that are not feasible due to the dynamics is 0.}
%and 
% given a path $\pathX \in \PathX$, we use
%by
%$\pathX^K$ its prefix of length $K+1$
 A \emph{strategy} of System~\eqref{eq:sys} is a function $\policy_x: \PathX \to U$ that assigns a control $u$ to each finite trajectory $\pathX$. 
Given $x\in\reals^n$, $u\in U$, the \emph{transition kernel} $T:\mathcal{B}(\reals^n)\times \reals^n\times U \rightarrow [0, 1]$
of System~\eqref{eq:sys} assigns the probability
$T(B\mid x,u) = \int_W \mathds{1}_{B}(f(x,u,w))P_W(dw)$, where the indicator function $\mathds{1}_B(x) = 1$ if $x \in B$, and $0$ otherwise,
to each Borel set $B\in\mathcal{B}(\reals^n)$. For a strategy $\policy_x$ and an initial condition $x_0\in\reals^n$, the transition kernel defines a unique probability measure $P_{x_0}^{\policy_x}$ over the trajectories of System~\eqref{eq:sys} \citep{bertsekas1996stochastic}.
%\ig{can we define a probability on $\PathX$? (remember that the length of the paths might be different)}  \LL{It is a bit informal the way it is written right now, as you either fix the path length or consider infinite paths and talk about different finite sub-paths using the Cylinder sigma algebra. I would like to avoid to go there, as it will take space }
%\ig{If enough space, make this more formal} \luca{Being a conference version and being this standard material, I would not go super formal. Otherwise, if we are extremely formal in here, we need to be it everywhere.}
In this way, $P_{x_0}^{\policy_x}[\pathXbold(k) \in B]$ denotes the probability that $\x_k$ belongs to the set $B\in \mathcal{B}(\reals^n)$ when following strategy $\policy_x$ from initial state $x_0$. 
In this work, we are interested in the temporal behavior of System~\eqref{eq:sys} w.r.t. a bounded (\emph{safe}) set $X\in \mathcal{B}(\reals^n)$ and a set of regions of interest $R_\text{int}% := \{r_1,\dots,r_{|R_\text{int}|}\}
$, with $r\subseteq X$ and $r\in \mathcal{B}(\reals^n)$ for all $r\in R_\text{int}$. We denote by $r_\text{unsafe} = \reals^n\setminus X$ the unsafe region. We consider a set $AP := \{\Prop_1,\dots,\Prop_{|AP|-1}, \Prop_\text{unsafe}\}$ of \emph{atomic propositions}, and associate a subset of atomic propositions to each region $r\in R_\text{int}\cup \{r_\text{unsafe}\}$. We define the \emph{labeling function} $L:\reals^n\rightarrow 2^{AP}$ as the function that maps each state $x\in \reals^n$ to the atomic propositions that are true in the region where $x$ lies, e.g., if we associate $\{\Prop_1\}$ to region $r_1$, we conclude that $\Prop_1$ is \textit{true} at $x$, denoted $\Prop_1 \equiv \top$, if $x\in r_1$. In consequence, each trajectory $\pathX= x_0 \xrightarrow{u_0} \ldots \xrightarrow{u_{K-1}} x_K$
results in the (observation) \emph{trace} 
$\rho = \rho_0\dots\rho_K, $
where $\rho_k := L(x_k)$. %for all $k\in\{0,\dots,K\}$. 

In order to formally characterize behaviors of System~\eqref{eq:sys}, we use \emph{linear temporal logic over finite traces} (\LTLf) \citep{de2013linear}, which generalizes Boolean logic to temporal behaviors.
%\ml{this last part of the sentence doesn't make sense.}\ig{what about now?}
%is a formal language commonly employed to express finite behaviors.
An \LTLf property $\varphi$ is a logical formula defined over atomic propositions $AP$ using Boolean connectives  ``negation'' ($\neg$) and ``conjunction'' ($\land$), and the temporal operators ``until'' ($\luntil$) and ``next'' ($\bigcirc$). The syntax of formula $\varphi$ is recursively defined as
%
    % \begin{align*}
    %     \varphi := \top \mid \Prop \mid \neg\varphi \mid \varphi_1\land\varphi_2 \mid \bigcirc\varphi \mid \varphi_1\luntil\varphi_2 
    % \end{align*}
    %
    $\varphi := \top \mid \Prop \mid \neg\varphi \mid \varphi_1\land\varphi_2 \mid \bigcirc\varphi \mid \varphi_1\luntil\varphi_2,$
    where $\Prop\in AP$ and $\varphi_1,\varphi_2$ are also \LTLf formulas.
%
The temporal operators ``eventually'' ($\Diamond$) and ``globally'' ($\Box$) are derived from the above syntax as  $\Diamond \varphi := \top\luntil\varphi$ and $\Box \varphi := \neg\Diamond(\neg\varphi)$.
\LTLf formulae are semantically interpreted over finite traces \citep{de2013linear}. We say a trajectory $\pathX$ satisfies a formula $\varphi$, i.e., $\pathX \models \varphi$, if some prefix of its trace $\rho$ satisfies $\varphi$.
 

% First note that, given a strategy of System~\eqref{eq:sys}, satisfaction of an \LTLf formula is probabilistic. Secondly, in our setting, the distribution of the disturbance is unknown. Our goal is to leverage data samples to synthesize a strategy which guarantees that System~\eqref{eq:sys} satisfies a given \LTLf formula with high probability. Note that the synthesized strategy also needs to account for the learning gap caused by the lack of knowledge of $P_W$. Now we formalize the problem.
%

Our goal is to synthesize a strategy for System~\eqref{eq:sys} to ensure satisfaction of a given \LTLf formula $\varphi$. However, note that (i) under a given strategy, the satisfaction of $\varphi$ is probabilistic, and (ii) in our setting, the distribution of the disturbance is unknown. Hence, we aim to leverage data samples to generate a strategy that guarantees System~\eqref{eq:sys} satisfies $\varphi$ with high probability. Furthermore, note that the synthesized strategy must account for the learning gap due to the lack of knowledge of $P_W$. 
% Now, we formalize the problem.

\begin{problem}
    \label{prob:Syntesis}
    %
    Consider stochastic System~\eqref{eq:sys}, a set $\{\hat\w^{(i)}\}_{i=1}^N$ of $N$ i.i.d. samples from $P_W$, a bounded set $X\in\mathcal{B}(\mathbb{R}^n)$ on which Assumption~\ref{ass:lipschitz} holds, and an \LTLf formula $\varphi'$ defined over the regions of interest $R_\text{int}$. Given a confidence level $1-\alpha \in (0,1)$, synthesize a strategy $\sigma_x$ and a high probability bound function $\underline p: X \rightarrow [0, 1]$ such that, with confidence at least $1-\alpha$, for every initial state $x_0\in X$, $\sigma_x$ guarantees that the probability that the paths $\pathX \in \PathX$ satisfy $\varphi := \varphi' \land \Box \neg \Prop_\text{unsafe}$ while remaining in $X$ is lower bounded by $\underline p(x_0)$, i.e.,
      $P_{x_0}^{\sigma_x}[\pathX \models \varphi] \ge \underline p(x_0)$.
\end{problem}

% We highlight that the noise distribution $P_W$ is unknown, and no assumptions are imposed on this one. Instead, since only samples are available, the guarantees required for the closed-loop system shall hold with a \emph{confidence}. This confidence is related to the probability that the $N$ samples are representative of $P_W$, and is interpreted in the frequentist sense: if the process of obtaining the $N$ samples from $P_W$ and synthesizing the strategy is repeated an infinite number of times, the result $P_{x_0}^{\sigma_x}[\pathX \models \varphi \land \Box \neg \Prop_\text{unsafe}] \ge \underline p(x_0)$ for all $x_0\in X$ will hold at least in a fraction of $1-\alpha$ of the total cases.

% \noindent
We remark that $P_W$ is unknown, and no assumptions are imposed on it. Instead, since only samples are available, the probabilistic satisfaction guarantees must hold with a \emph{confidence}, related to the probability that the $N$ samples are representative of $P_W$, and interpreted in the frequentist sense: if the process of sampling $N$ times from $P_W$ and synthesizing $\sigma_x$ is repeated infinitely many times, the condition $P_{x_0}^{\sigma_x}[\pathX \models \varphi] \ge \underline p(x_0)$ for all $x_0 \in X$ holds in at least $1-\alpha$ of the cases.




\paragraph*{Overview of the approach} 
% Given the uncountable nature of the state-space of System~\eqref{eq:sys} and the fact that $P_W$ is unknown, solving Problem \ref{prob:Syntesis} exactly is generally infeasible. Consequently, since the objective is not to find a strategy that maximizes the satisfaction probability, we adopt an abstraction-based approach.  This approach yields a strategy along with a conservative, but sound, high-probability bound for every initial state. The abstraction is an uncertain Markov decision process, which we learn from data.  It accounts for the learning gap, thereby guaranteeing that the obtained strategy is robust against this uncertainty.

% First, in Section \ref{sec:preliminaries}, we briefly introduce our abstraction class: uncertain Markov decision processes (UMDPs). In Section~\ref{sec:abstraction} we obtain a UMDP abstraction of System~\eqref{eq:sys} from the samples of the disturbance, which captures all behaviors of System~\eqref{eq:sys} with confidence $1-\alpha$. Next, in Section~\ref{sec:synthesis}, we synthesize a strategy for the abstraction via robust dynamic programming. This strategy (robustly) maximizes the probability that the abstraction satisfies the \LTLf specification. Section~\ref{sec:algorithm} describes an efficient algorithm to perform robust dynamic programming for our UMDP abstraction class. Finally, we refine the obtained strategy to System~\eqref{eq:sys}, in such a way that the closed-loop system is guaranteed to satisfy the \LTLf specification with a probability higher than the one obtained for the abstraction, with confidence $1-\alpha$. We empirically validate our approach through several case studies in Section~\ref{sec:case_studies}.


% First, in Section~\ref{sec:preliminaries}, we introduce our abstraction class, uncertain Markov decision processes (UMDPs). In Section~\ref{sec:abstraction}, we derive a UMDP abstraction of System~\eqref{eq:sys} from disturbance samples, capturing its behaviors with confidence $1-\alpha$. Section~\ref{sec:synthesis} presents a strategy synthesized via robust dynamic programming, maximizing the probability that the abstraction satisfies the \LTLf specification. In Section~\ref{sec:algorithm}, we describe an efficient algorithm for this synthesis. Finally, we refine the strategy for System~\eqref{eq:sys} to ensure the closed-loop system satisfies the specification with higher probability and confidence $1-\alpha$. Empirical validation is provided in Section~\ref{sec:case_studies}.

% Due to the uncountable state-space of System~\eqref{eq:sys} and the unknown disturbance distribution $P_W$, solving Problem \ref{prob:Syntesis} exactly is infeasible. Therefore, we adopt an abstraction-based approach, which allows generating a strategy along with a (conservative) high-probability bound for each initial state. The abstraction, an uncertain Markov decision process learned from data, accounts for the learning gap, ensuring the strategy is robust against uncertainty.

% In Section~\ref{sec:preliminaries}, we introduce uncertain Markov decision processes (UMDPs) as our abstraction class. In Section~\ref{sec:abstraction}, we derive a UMDP abstraction from disturbance samples, capturing the system’s behavior with confidence $1-\alpha$. Section~\ref{sec:synthesis} presents a strategy synthesized using robust dynamic programming, maximizing the probability that the abstraction satisfies the \LTLf specification. An efficient algorithm for synthesis is described in Section~\ref{sec:algorithm}. Finally, we refine the strategy for System~\eqref{eq:sys} to ensure the closed-loop system satisfies the specification with higher probability and confidence $1-\alpha$. Empirical validation is provided in Section~\ref{sec:case_studies}.

Given the uncountable nature of the state-space of System~\eqref{eq:sys} and $P_W$  being unknown, solving Problem \ref{prob:Syntesis} exactly is infeasible. Therefore, we adopt an abstraction-based approach, which provides a strategy along with a conservative, high-probability bound for every initial state. The abstraction is an uncertain MDP (UMDP) constructed from a finite partition of $X$. We learn the transition relations between regions using $f$ and disturbance samples, capturing the system's behavior with confidence $1-\alpha$.  
Our UMDP construction is specifically designed to tightly capture the learning uncertainty.
% Our construction of UMDP is specifically tuned to also tightly capture the learning uncertainty. 
Then, we devise a strategy synthesis algorithm based on robust dynamic programming to (robustly) maximize the probability of satisfying $\varphi$ on this UMDP.  Next, we refine this strategy to System~\eqref{eq:sys} such that it guarantees that the closed-loop system satisfies $\varphi$ with a probability higher than the one obtained for the abstraction with confidence $1-\alpha$. 











==> Sections/3_preliminaries.tex <==
\section{Preliminaries on Uncertain Markov Decision Processes}
\label{sec:preliminaries}

% An uncertain MDP (UMDP), also known as robust MDP, is a stochastic system that generalizes the MDP class by letting its transition probability distributions be uncertain, namely, they take values in a set \cite{iyengar2005robust,el2005robust,wiesemann2013robust}.
%\aabate{are we all happy with Robust MDP, or should we consider using Uncertain MDP (as per recent literature other than that listed) instead?} \ig{Personally, I definitely prefer Uncertain MDP}\luca{I am fine with uncertain MDPs.}

An uncertain MDP (UMDP), also known as a robust MDP, is a stochastic system that generalizes the MDP class by allowing its transition probability distributions to be uncertain, taking values from a set \citep{iyengar2005robust,el2005robust,wiesemann2013robust}.

\begin{definition}[Uncertain MDP]
\label{def:robust_mdp}
    A labeled uncertain Markov decision process (UMDP) $\M$ is a tuple $\M = (S,A,\Gamma,s_0,AP,L)$, where 
    $S$ and $A$ are finite sets of states and actions, respectively, $s_0 \in S$ is the initial state,
    % \begin{itemize}
        % \setlength\itemsep{0.1mm}
        % \item $S$ and $A$ are finite sets of states and actions, respectively, $s_0 \in S$ is the initial state,
        % \item $\Gamma = \{\Gamma_{s,a} \subseteq \mathcal{P}(S) : {s\in S, a\in A}\}$, where 
        % $\mathcal{P}(S)$ is the set of probability distributions over $S$, and $\Gamma_{s,a}$ is a nonempty set of transition probability distributions for state $s\in S$ and action $a \in A$,
        % \item $AP$ is a finite set of atomic propositions, and $L:S\rightarrow 2^{AP}$ denotes the labeling function.
    % \end{itemize}
    $\Gamma = \{\Gamma_{s,a} \subseteq \mathcal{P}(S) : {s\in S, a\in A}\}$, where $\mathcal{P}(S)$ is the set of probability distributions on $S$, and $\Gamma_{s,a} \neq \emptyset$ is the set of transition probability distributions for state $s\in S$ and action $a \in A$,
    $AP$ is a finite set of atomic propositions, and $L:S\rightarrow 2^{AP}$ is the labeling function.
\end{definition}

A \emph{strategy} of a UMDP $\M$ is a function $\policy: \Pathrmdp \rightarrow A$ that maps each finite path to the next action. We denote by $\Sigma$ the set of all strategies of $\M$. 
%Fixing a strategy $\policy\in\Setofpolicies$ restricts the set of transition probability distributions \ml{what do you mean by this?} of $\M$, which yields a set of Markov chains, or uncertain Markov chain. 
Given path $\pathrmdp \in \Pathrmdp$ and $\policy \in \Sigma$, the process evolves from $s_{k} = \last(\path)$ under $a_k = \policy(\pathrmdp)$ to the next state according to a distribution in $\Gamma_{s_k,a_k}$. This distribution is chosen by the adversary \citep{givan2000bounded}. Formally, an \emph{adversary} is a function $\adversary: S \times A \times \big(\naturals\cup \{0\}\big) \rightarrow \mathcal{P}(S)$ that maps each state $s_k$, action $a_k$, and time step $k\in\naturals\cup \{0\}$ to a transition probability distribution $\gamma\in\Gamma_{s_k,a_k}$, such that $s_{k+1} \sim \gamma$. We denote the set of all adversaries by $\Adversary$. Given an initial condition $s_0\in S$, a strategy $\policy\in\Setofpolicies$ and an adversary $\xi\in\Xi$, the UMDP collapses to a Markov chain
 % , and a unique probability distribution $Pr_{s_0}^{\policy,\xi}$ is induced on its paths.
with a unique probability distribution $Pr_{s_0}^{\policy,\xi}$ over its paths.
 
\iffalse

\subsection{Concentration Inequalities}

\ig{Does it make sense to introduce here the learning techniques we will use use? I feel like doing so will take more space}\luca{It depends but if you just rely on concentration inequalities, then no need}

\fi

==> Sections/4_proposed_approach.tex <==
\section{Data-driven UMDP Abstraction}
\label{sec:abstraction}
%We solve Problem~\ref{prob:Syntesis} in two steps: first,
In this section, we construct a UMDP $\M$, whose path probabilities are guaranteed to encompass the probabilities of System~\eqref{eq:sys}'s trajectories with confidence $1-\alpha$
. 
%After that, in Section~\ref{sec:synthesis}, we synthesize a strategy for System~\ref{eq:sys} and lower-bound the probability that the closed-loop system satisfies the \LTLf formula $\varphi$.
%
We define the set of states $S$ of $\M$ as follows. Let $R := \{r_1,\dots, r_{|R|}\}$ be a finite partition of the continuous state-space $\mathbb{R}^n$ into non-overlapping, non-empty regions, which respects the regions of interest $R_\text{int}$ and the safe set $X$, and such that $r\in\mathcal{B}(\reals^n)$ for all $r\in R$. We let region $r_{|R|} := r_\text{unsafe}$ represent the unsafe set. 
%\ml{Why don't we simply say: Let $R := \{r_1,\dots, r_{|R|}\}$ be a finite partition continuous state-space $\mathbb{R}^n$ into non-overlapping, non-empty regions such that $\bigcup_{i=1}^{|R|-1} r_i = X$ and $r_{|R|} =\reals^n\setminus X$.} \ig{Isn't the first condition implied by the word ''partition"}
We assign each region $r \in R$ to a state $s \in S$ in the abstraction $\M$ through the bijective map $J: R \rightarrow S$, which ensures that $J^{-1}(s)  = r \in R$ is unique. For simplicity, we abuse the notation and also say $J(x) = s$ if $x \in r$ with $J(r) = s$.
We define the action set $A$ of $\M$ as $A :=U$. With a slight abuse of language, we also denote by $L$ the labeling function of $\M$, which maps each state $s\in S$ to the atomic propositions that hold at $x\in r = J^{-1}(s)$. 
%\ml{so the partition $R$ respects the regions of interest.}\ig{added that part before}
Next, we define the set of transition probability distributions of the abstraction. To that end, we begin by stating the following proposition, whose proof follows from \citep[Eq.12]{badings2023probabilities}\footnote{The measurability of the events in  \eqref{eq:tp_bounds} is formally proved in the supplementary material \citep{supp}.}, which gives uniform bounds in the probabilities that System~\eqref{eq:sys} transitions from each point $x$ in some region $r\in R$ to some region $\tilde r \in \mathcal{B}(\reals^n)$.

\begin{proposition}
    \label{prop:tp_bounds}
    Given a region $r\in R$, an action $a\in A$ and a realization $w\in W$ of $\w$, denote by $\text{Reach}(r,a,w) := \{f(x,a,w) : x\in r\}$ the reachable set of $r$ under $a$ and $w$. %Let $\{r_i\}_{i\in I}$ be an arbitrary number of regions from $R$, with indices in some set $I\subseteq\naturals$, and denote the union of these regions by $\tilde r$.
    % Let $\tilde r\in\mathcal{B}(\reals^n)$. 
    Then, the probability of transitioning from each state $x\in r$ to region $\tilde r \in \mathcal{B}(\reals^n)$ under action $a\in A$ is bounded by
    %
    \begin{align}
\label{eq:tp_bounds}
    P_W(\{w : \text{Reach}(r,a,w)\subseteq \tilde r \}) \le T(\tilde r \mid x, a) \le P_W(\{w : \text{Reach}(r,a,w) \cap \tilde r \neq \emptyset \})
\end{align}
\end{proposition}
%
\iffalse
\begin{proof}
    By the logic of \citep[Eq.12]{badings2023probabilities}
    %\ml{didn't John also prove this?}\ig{he did, but he didn't talk about measurability, and you can't define the probability if it is not measurable}
    , we have that, for all $x\in r$,
    $\text{Reach}(r,a,w)\subseteq \tilde r \implies f(x,a,w_k(\omega))\in \tilde r \implies \text{Reach}(r,a,w)\cap \tilde r \neq \emptyset.$
%
% \begin{align*}
    % \text{Reach}(r,a,w)\subseteq \tilde r \implies f(x,a,w_k(\omega))\in \tilde r \implies \text{Reach}(r,a,w)\cap \tilde r \neq \emptyset
% \end{align*}
%
\iffalse
In practice we are interested in the cases when the reachable set intersects $r$ or is a subset of $r$, rather than $\tilde r$ itself. It is evident that
%
\begin{align*}
    \text{Reach}(r,a,w_k(\omega))\subseteq r \implies f(x,a,w_k(\omega))\in \tilde r \implies \text{Reach}(r,a,w_k(\omega))\bigcap r \neq \emptyset.
\end{align*}
%
\fi
Then, \eqref{eq:tp_bounds} follows from mensurability of these events, which we prove in the supplementary material \citep{supp}.
%
\end{proof}
\fi
% 
%The proof of measurability of the events in \eqref{eq:tp_bounds} is provided in the supplementary material \ml{CITE}.
% Below, we leverage the samples from $\w$ to find data-driven bounds that contain the ones in \eqref{eq:tp_bounds}, and use these bounds to define the set of transition probability distributions of $\M$.
Below, we use the samples of $\w$ to derive data-driven bounds that contain the ones in \eqref{eq:tp_bounds} and leverage these bounds to define the set of transition probability distributions for $\M$.

\iffalse

\subsection{Measurability of the events in \eqref{eq:tp_bounds}}
\label{sec:measurability}
%\luca{This can go in the Appendix as it is natural to me that the events are measurable. I would just add a sentence in here saying: note that the probabilities in 2 are well defined, as formally proved in Appendix \ref{}. } \ig{I agree that the paper would flow better like that. I'm concerned about space though: the appendix counts towards the 10 page limit...}

\ml{move this to the supplementary material}

Consider the closed set-valued function $w\mapsto g(w) :=\text{Reach}(r,a,w)$, for all $w\in W,$ and let $B(0,\epsilon) \subset \reals^n$ denote the $\epsilon$-ball centered at the origin. We begin by stating the following technical lemma:
%
\begin{lemma}
\label{eq:lemma_epsilon_reach_set}
    For all $w\in W$, $\epsilon >0$, there exists a $\delta >0$ such that for all $w'\in W$ with $\|w - w'\| < \delta$, $g(w') \subseteq g(w)\oplus B(0,\epsilon)$ holds.
\end{lemma}
%
\begin{proof}
Pick $w\in W$, $\epsilon >0$, and let $\delta = \epsilon/L(r,a)$. We want to show that for all $w'\in W$ with $\|w - w'\| < \delta$ and $y'\in g(w')$ there exists a $y \in g(w)$ that is only $\epsilon$-apart. Then the statement in the proposition follows. Define $x$ such that $f(x,a,w') = y'$, which is possible by definition of $g(w')$, and let $y = f(x,a,w)$, which implies $y\in g(w)$. By Lipschitz continuity of $f$, we obtain that $\|y-y'\| = \|f(x,a,w) - f(x,a,w')\| \le L(r,a)\|w-w'\| < \epsilon$. Thus the proof is concluded.
\end{proof}
%
\begin{proposition}
    The probability bounds in \eqref{eq:tp_bounds} are well-defined
\end{proposition}
%
\begin{proof}
    The proof only requires establishing that the events in \eqref{eq:tp_bounds} are measurable. Denote by $\mathcal{F}$, $\mathcal{G}$ and $\mathcal{K}$ respectively the sets of all closed, open and compact subsets of $\mathbb{R}^n$ with respect to the usual topology. Consider the Fell topology $\mathcal{T}(\mathcal{F})$ on $\mathcal{F}$, i.e. the one generated by the sets
%
\begin{align*}
    \mathcal{F}^K := \{F \in \mathcal{F}(\mathbb{R}^n) : F \bigcap K = \emptyset\}\qquad\text{and}\qquad
    \mathcal{F}_G := \{F \in \mathcal{F}(\mathbb{R}^n) : F \bigcap G \neq \emptyset\},
\end{align*}
%
for all $G\in\mathcal{G}$ and $K\in\mathcal{K}$. Denote by $\mathcal{B(\mathcal{F})}$ the Borel $\sigma$-algebra on $(\mathcal{F}, \mathcal{T})$. Denote also by $\mathcal{T}(W)$ the usual topology on $W$ and by $\mathcal{B}(W)$ the Borel $\sigma$-algebra on $W$. For simplicity, assume that $\text{Reach}(r,a,w)$ is closed and note that if it is not, we can always consider its closure without compromising the soundness of the approach. First, we establish that the function $g$ is $(W, \mathcal{B}(W))$-$(\mathcal{F},\mathcal{B}(\mathcal{F}))$ measurable by proving a sufficient condition, namely, upper semi-continuity of $g$: $g$ is upper semi-continuous if $g^-(K) := \{w\in W : g(w)\bigcap K \neq \emptyset\}$ is closed on $(W,\mathcal{T}(W))$ for all $K\in\mathcal{K}$. We proceed by contradiction: assume that $g^-(K)$ is not closed for some $K\in\mathcal{K}$. Then, there must exist a $w_\infty\in W\setminus g^-(K)$ and a sequence $\{w_n\}_{n\in\naturals} \subset g^-(K)$ that converges to $w_\infty$. Since $K$ and $g(w_\infty)$ are closed and non-intersecting, there exists $\epsilon>0$ such that $(g(w_\infty)\oplus B(0,\epsilon))\bigcap K = \emptyset$. %It is straightforward to note that $w_\infty$ must belong to the boundary of $g^-(K)$.
By convergence of $\{w_n\}_{n\in\mathbb{N}}$, for every $\delta >0$ $\exists N \in \mathbb{N}$ such that $\|w_\infty-w_N\| < \delta$. This implies, by Lemma~\ref{eq:lemma_epsilon_reach_set}, that we can choose $N$ large enough so that we ensure, $g(w_N) \subseteq g(w_\infty)\oplus B(0,\epsilon)$. It follows that $g(w_N)\bigcap K \subseteq (g(w_\infty)\oplus B(0,\epsilon))\bigcap K = \emptyset$, which proves that $w_N\notin g^-(K)$, being this result a contradiction. Therefore $g^-(K)$ is closed in $(W,\mathcal{T}(W))$ for all $K\in\mathcal{K}$, making $g$ upper-semicontinuous and measurable, i.e., $w \mapsto \text{Reach}(r,a,w)$ is a well-defined random set \cite{molchanov2005theory}. Finally, since $\tilde r$ can be written as the union of countably many
closed sets, the events $\{F \in \mathcal{F} : F \bigcap \tilde r \neq \emptyset\}$ and $\{F \in \mathcal{F} : F \subseteq \tilde r \}$ are measurable, i.e., they belong to $\mathcal{B}(\mathcal{F})$, which implies measurability of $\{\omega \in \Omega : \text{Reach}(r,a,w) \bigcap \tilde r \neq \emptyset\}$ and $\{\omega \in \Omega : \text{Reach}(r,a,w) \subseteq \tilde r\}$, thus concluding the proof.
\end{proof}

\fi



\subsection{Data-Driven Transition Probability Bounds}
\label{sec:data_driven_bounds}

We now construct the sets $\Gamma_{s,a}$ of transition probability distributions of the abstraction by leveraging the samples from $\w$. Specifically, in our abstraction, each set $\Gamma_{s,a}$ is defined by: (i) interval bounds on the probability of transitioning to each state $s'\in S$, (ii) interval bounds on the probability of transitioning to a cluster of states in $2^S$, and (iii) a bound on the probability of transitioning to states within the reachable set of the learned support of $P_W$.  Notably, (ii) and (iii) distinguish our construction from prior work, which relies solely on (i). As a result, our UMDP incorporates additional constraints, leading to tighter uncertainty sets. This yields less conservative probabilistic guarantees, as shown in the case studies. To derive the bounds (i)-(iii), we use Proposition~\ref{prop:tp_bounds}, samples from $\w$, and two well-known concentration inequalities. Proposition~\ref{prop:hoeffding} %Proposition~\ref{prop:hoeffding} 
enables us to compute bounds on transition probabilities between regions, which we later use to obtain bounds in (i)-(ii).

\begin{proposition}
\label{prop:hoeffding}
    Consider the set $\{\boldsymbol{\hat w}^{(i)}\}_{i=1}^N$ of i.i.d. samples from $\w$. Pick $r\in R$, $a\in A$, $\tilde r \in \mathcal{B}(\reals^n)$ and $\beta \in(0, 1)$, and let $\epsilon = \sqrt{\log(2/\beta)/(2N)} >0 $. Then, with confidence at least $1-\beta$ we have 
    that, for all $x\in r$,
    %
    \begin{subequations}
        \label{eq:data_driven_bounds}
        \begin{align}
            T(\tilde r\mid x, a) &\ge \underline P(r, a)(\tilde r) := \frac{1}{N} \Big| \{i\in\{1,\ldots,N\}:\text{Reach}(r,a, \boldsymbol{\hat w}^{(i)})\subseteq \tilde r \} \Big| - \epsilon \label{eq:data_driven_bounds_lower}\\
            T(\tilde r\mid x, a) &\le \overline P(r, a)(\tilde r) := \frac{1}{N} 
            \Big| \{i\in\{1,\ldots,N\}:\text{Reach}(r,a, \boldsymbol{\hat w}^{(i)})\cap \tilde r \neq \emptyset\} \Big| + \epsilon. \label{eq:data_driven_bounds_upper}
        \end{align}
    \end{subequations}
 %
\end{proposition}
%
\begin{proof}
Consider the lower bound in \eqref{eq:tp_bounds}. Denote $E := \{w\in W : \text{Reach}(r,a,w)\subseteq \tilde r \}$ and note that
%
%\begin{align*}
    $T(\tilde r\mid x, a) \ge P_W(E) = \mathbb{E}_{P_W}[\mathds{1}_{E}(\w)]$
%\end{align*}
%
for all $x\in r$. Therefore applying Hoeffding's inequality to the random variable $\frac{1}{N}\sum_{i=1}^N\mathds{1}_{E}(\boldsymbol{\hat w}^{(i)})$ yields 
%
%\begin{align*}
    $P_W^N[P_W(E)  \ge \frac{1}{N}\sum_{i=1}^N\mathds{1}_{E}(\boldsymbol{\hat w}^{(i)}) - \epsilon] \ge 1-\beta/2$,
%\end{align*}
%
with $\epsilon = \sqrt{\log(2/\beta)/(2N)}$. Thus, the first expression in ~\eqref{eq:data_driven_bounds} holds 
\iffalse
%
\begin{align*}
    T(\tilde r\mid x, a)\ge P_W(E) \ge \frac{1}{N}\sum_{j=1}^N\mathds{1}_{E}(\boldsymbol{\hat w}^{(j)}) - \epsilon
\end{align*}
%
\fi
for all $x\in r$ with confidence $1-\beta/2$. Employing a similar argument, we obtain a similar result for the second expression in ~\eqref{eq:data_driven_bounds}.
\iffalse
%
\begin{align*}
    T(\tilde r\mid x, a)\le \frac{1}{N}\sum_{j=1}^N\mathds{1}_{E}(\boldsymbol{\hat w}^{(j)}) - \epsilon
\end{align*}
%
\fi
Combining both results via the union bound, we obtain the result.
%
\end{proof}
%
%For practical reasons, instead of checking if $\text{Reach}(r,a,w_k(\omega^{(i)}))\subseteq \tilde r$, we check whether or not some set overapproximating $\text{Reach}(r,a,w_k(\omega^{(i)}))$ is contained in $r$. It is easy to verify that if this is the case, then $\text{Reach}(r,a,w_k(\omega^{(i)}))\subseteq \tilde r$, and thus we obtain a sound lower bound to $T(\tilde r\mid x, a)$.
%The same reasoning yields a lower bound on $T(\tilde r\mid x, a)$ with confidence $1-\beta/2$. Again, for practical reasons, we check whether or not some set overapproximating $\text{Reach}(r,a,w_k(\omega^{(i)}))$ intersects $r$, which is a necessary condition for $\text{Reach}(r,a,w_k(\omega^{(i)}))\bigcap \tilde r$, and thus we obtain a sound upper bound to $T(\tilde r\mid x, a)$.

%\ml{explain what this proposition allows you to do.  It takes care of transition probabilities between which regions?}

\noindent
% Proposition~\ref{prop:hoeffding} enables us to compute bounds in the probability of transitioning between regions $r$ and $\tilde{r}$ under action $a$.


\begin{remark}
    The complexity of computing the bounds in \eqref{eq:data_driven_bounds} is proportional to $N$, which is typically high to obtain tight bounds. To reduce this complexity, we cluster the $N$ samples from $\w$ into $N_c \ll N$ clusters, each with center $c_j$ and diameter $\phi_j$. Substituting the sets $\text{Reach}(r,a,\boldsymbol{\hat w}^{(j)})$ in \eqref{eq:data_driven_bounds} by $\{f(x,a,w) \in \reals^n : x\in r, \|w - c_j\| \le \phi_j/2)\}$, it is evident that Proposition~\ref{prop:hoeffding} still holds, with relaxed bounds. Note that this clustering induces a partition on $W$, allowing to overapproximate the sets $\{f(x,a,w) \in \reals^n : x\in r, \|w - c_j\| \le \phi_j/2)\}$ as shown by \cite{skovbekk2023formal}.
\end{remark}

%\subsection{Learning a Confidence Region for the Noise}

Next, we estimate the support of $P_W$ in (iii). Including this information into $\M$ tightens the sets $\Gamma_{s,a}$ of transition probability distributions, thus yielding a less conservative abstraction.
%Furthermore, it also helps reducing the size of the abstraction.
%\ml{motivate and explain why this is needed and how it improves the abstraction.}

\begin{proposition}[Confidence Region {\citep{tempo2013randomized}}]
\label{prop:confidence}
%Let $(Y,\mathcal{B}(Y),P)$ be a probability space, with $Y\subseteq\mathbb{R}$, and consider the sequence $\{y^{(i)}\}_{i = 1}^N$ $P$-distributed i.i.d. random variables. 
Let $\hat c = \max\{\|\boldsymbol{\hat w}^{(1)}\|, \dots, \|\boldsymbol{\hat w}^{(N)}\|\}$.
%Let $h:Y\rightarrow \mathbb{R}_{\ge 0}$ be a measurable.
Then, for any $\epsilon_c, \beta_c >0$ and 
%
%\begin{align*}
    $N \ge \log{(1/\beta_c)}/\log{(1/(1-\epsilon_c}))$,
%\end{align*}
%
it holds, with a confidence greater than $1-\beta_c$ with respect to the random choice of $\{\boldsymbol{\hat w}^{(i)}\}_{i = 1}^N$, that 
%
%\begin{align*}
    $P_W(\{w\in W : \|w\| \le \hat c\}) \ge 1 - \epsilon_c$.
%\end{align*}
\end{proposition}
%
\iffalse
\begin{proof}
    Since $\|\cdot\|$ is a measurable function, a direct application of \cite{tempo2013randomized}[Theorem 9.1] to the random variables $\|y\|\, |y^{(1)}\|, \dots, \|y^{(N)}\|$ yields the
\end{proof}
\fi

We denote the learned confidence region for $w$ by $\widehat W := \{w\in W : \|w\| \le \hat c\}$, which contains at least $1-\epsilon_c$ probability mass from $P_W$ with a confidence greater than $1-\beta_c$. We also define $\widehat{\text{Post}}(s,a) := \{J(f(x,a,w))\in S : x\in J^{-1}(s), w\in \widehat W\}$ for each $s\in S$, $a\in A$ to be the set of abstract states that can be reached from region $J^{-1}(s)$ and under some noise realization $w\in\widehat W$.


We now have all the components needed to define our abstraction. 
Intuitively, we leverage a two-layer discretization: a fine one represented by $S$ and a coarse one formed by clustering the elements of $S$ (see Figure~\ref{fig:figure}). 
Let $Q \subseteq 2^S$ be this clustering, which is non-overlapping and $\bigcup_{q \in Q} q = S$. $Q$ is crucial for obtaining non-zero lower-bound transition probabilities in \eqref{eq:data_driven_bounds_lower}, as $\text{Reach}(r, a, \hat{\w}^{(i)})$ often cannot be contained within a single small region but can be captured by a cluster of them (see Figure~\ref{fig:figure}). %the supplementary material in \citep{supp}).
We also leverage the learned support $\widehat W$ of $P_W$ to impose the constraint that the successor state of a given $(s,a)$ pair lies on some region with high probability. As described in \citep{supp}, this constraint is key for our approach to be effective. Note that varying $R$ and $Q$ yields a different abstraction, which makes them hyperparameters. We now formally define our abstraction.

\begin{wrapfigure}{R}{0.34\textwidth}
    \vspace{-10mm}
    \begin{minipage}{0.34\textwidth}
        \begin{figure}[H]
            \includegraphics[width=\textwidth]{images/l4dc2025_UMDP.drawio-4c.pdf}
            \caption{ Illustration of the sets in Def.~\ref{def:robust_mdp}. $C(s,a) = \{q_1,q_2,q_3,q_4\}$, and each $q_i$ contains $4$ states. The probability that the successor state of $s=J(r)$ under action $a$ will be in $C(s,a)$ is higher than $1-\epsilon$. Note that the reachable sets corresponding to $\boldsymbol{\hat w}^{(2)}$ and $\boldsymbol{\hat w}^{(3)}$ are contained in $q_3$ and $q_4$, respectively, but no single regions in the fine partition contains them completely.}
            \label{fig:figure}
        \end{figure}
    \end{minipage}
    \vspace{-5mm}
\end{wrapfigure}

\begin{definition}[UMDP Abstraction]
    \label{def:umdp abstraction}
    % Let $Q(s,a)\subset 2^S$, where each $q'\in Q(s,a)$ is a set of aggregate states of the abstraction, or \emph{cluster}, such that its union $C(s,a) := \bigcup_{q'\in Q(s,a)} q'$ covers $\widehat{\text{Post}}(s,a)$. We define the UMDP abstraction of System~\eqref{eq:sys} as $\M = (S,A,s_0,\Gamma,AP,L)$, with, for all $s\in S$ and $a\in A$,
    Let $Q\subseteq 2^S$ be a non-overlapping clustering of $S$ and, for all $s\in S\setminus\{s_{|S|}\}$, $a\in A$, let $Q(s,a) \subseteq Q $ be the subset 
    that covers $\widehat{\text{Post}}(s,a)$, i.e., $\widehat{\text{Post}}(s,a)$ is contained in $C(s,a) := \bigcup_{q\in Q(s,a)} q$. We define the UMDP abstraction of System~\eqref{eq:sys} as $\M = (S,A,s_0,\Gamma,AP,L)$, with, $\forall s\in S\setminus\{s_{|S|}\}$ and $\forall a\in A$,
    \begin{align}
    \label{eq:Gamma}
        \Gamma_{s,a} := \big\{ & \gamma \in \mathcal{P}(S) : \underline P(r_s, a)(r_{s'})  \le \gamma(s') \le \overline P(r_s, a)(r_{s'}) \quad\;\;\; \forall s' \in C(s,a), \nonumber \\
        &\; \underline P(r_s, a)(r_{q'}) \le \sum_{s'\in q'}\gamma(s') \le \overline P(r_s, a)(r_{q'}) \:\; \forall q' \in Q(s,a), \!\!\sum_{s'\in C(s,a)} \!\!\!\! \gamma(s') \ge 1 - \epsilon_c \big\}, 
    \end{align}
%
where $\underline P, \overline P$ are defined in \eqref{eq:data_driven_bounds},
%
\iffalse
\begin{align}
\label{eq:conditions}
    \begin{split}
        \underline{P}(s,a)(s') &:= \frac{1}{N} |\{i\in\{1,\ldots,N\}:\text{Reach}(r_s,a, \boldsymbol{\hat w}^{(i)})\subseteq r_{s'} \}| - \epsilon\\
        \overline{P}(s,a)(s') &:= \frac{1}{N} |\{i\in\{1,\ldots,N\}:\text{Reach}(r_s,a, \boldsymbol{\hat w}^{(i)})\bigcap r_{s'} \neq \emptyset\}| + \epsilon,\\
        \underline{P}(s,a)(q') &:= \frac{1}{N} |\{i\in\{1,\ldots,N\}:\text{Reach}(r_s,a, \boldsymbol{\hat w}^{(i)})\subseteq \tilde r_{q'} \}| - \epsilon\\
        \overline{P}(s,a)(q') &:= \frac{1}{N} |\{i\in\{1,\ldots,N\}:\text{Reach}(r_s,a, \boldsymbol{\hat w}^{(i)})\bigcap \tilde r_{q'} \neq \emptyset\}| + \epsilon,
    \end{split}
\end{align}
%
\fi
% $r_{s'} = J^{-1}(s')$  for all $s'\in C(s,a)$, $\tilde r_{q'} = \bigcup_{s'\in q'} J^{-1}(s')$, for all $q'\in Q(s,a)$.
$r_{s'} = J^{-1}(s')$, and $r_{q'} = \bigcup_{s'\in q'} J^{-1}(s')$, and $\Gamma_{s_{|S|},a} = \{\delta_{s_{|S|}}\}$ for all $a\in A$, where $\delta_{s_{|S|}}$ denotes the Dirac measure located at $s_{|S|}$.
%
\end{definition}

\iffalse
\ig{Some results. Corollary maybe??}

Let $\M = (S,A,\Gamma,\text{AP},L)$ be a UMDP with
%
\begin{align}
\label{eq:conditions_rmdp}
    \sum_{s'\in S}\underline P(s,a)(s') \le 1 \quad &\\
    \sum_{s'\in S}\overline P(s,a)(s') \ge 1 \quad &\\
    \underline P(s,a)(q') \le \sum_{s'\in q'}\overline P(s,a)(s') \quad &\text{for all}\: q'\in Q(s,a)\\
    \overline P(s,a)(q') \ge \sum_{s'\in q'}\underline P(s,a)(s') \quad &\text{for all}\: q'\in Q(s,a)\\
    \sum_{s'\in C(s,a)} \overline P(s,a)(s') \ge 1 - \epsilon_c \quad&\\
    q' \subseteq C(s,a) \quad& \text{for all}\: q'\in Q(s,a)\\
    C(s,a) \supseteq \widehat{\text{Post}}(s,a), \quad&
\end{align}
%
for all $s\in S, a\in A$.

\fi


Note that, by making the unsafe state absorbing, we embed the safety part $\Box \neg \Prop_\text{unsafe}$ of $\varphi$ into $\M$, since a path of $\M$ satisfies $\varphi'$ only if it remains in $X$. In Theorem~\ref{theorem:soundness}, we establish that the UMDP $\M$ is a sound abstraction of System~\eqref{eq:sys}, i.e., that $\M$ captures all $1$-step behaviors of System~\eqref{eq:sys}.

% \aabate{why a Lemma? is it used to prove something else?} \ig{Yes, we rely on this Lemma to prove Theorem \ref{thm:strategy_synthesis}, i.e., that strategy synthesis gives us a sound lower bound in the probability that System~\eqref{eq:sys} satisfies $\varphi$}



\begin{theorem}[Soundness of UMDP Abstraction]
\label{theorem:soundness}
    For all $s\in S\setminus\{s_{|S|}\}$, $a\in A$, $x\in J^{-1}(s)$, $s'\in S$ define $\gamma_x\in\mathcal{P}(S)$ as
    %
    %\begin{align*}
        $\gamma_x(s') := T(J^{-1}(s')\mid x,a)$ 
    %\end{align*}
    %
    for all $s'\in S$. Then, $\gamma_x\in \Gamma_{s,a}$ for all $s\in S\setminus\{s_{|S|}\}$, $a\in A$, with confidence of at least $1-\alpha$, where $\alpha = \beta_c + \big( \sum_{s\in S\setminus\{s_{|S|}\}, a\in A} |C(s,a)| + |Q(s,a)| \big)\beta$.
\end{theorem}
%
The proof of Theorem~\ref{theorem:soundness} is provided in the supplementary material~\citep{supp}. Note that $|C(s,a)|$ and $|Q(s,a)|$ depend on the samples from $P_W$ trough $\widehat W$ (see Proposition~\ref{prop:confidence}). However, the expression for $\alpha$ in Theorem~\ref{theorem:soundness} follows from a union bound argument, which holds only if the number of transitions $\sum_{s\in S\setminus\{s_{|S|}\}, a\in A} |C(s,a)| + |Q(s,a)|$ is deterministic. We solve this issue by first estimating this number. Then, given $\alpha, \beta_c, \epsilon_c$ and $N$, we solve for $\beta$ and $\epsilon$, and obtain the corresponding abstraction $\M$. Finally, we check that the actual number of transitions does not exceed the estimated one, guaranteeing that $\M$ is sound by Theorem~\ref{theorem:soundness}.
\iffalse
\begin{proof}
    By Proposition~\ref{prop:hoeffding} we have that $\underline P(s,a)(s') \le \gamma_x(s')$ with confidence $1-\beta/2$ pointwisely for all $s'\in C(s,a)$, and similarly for the upper bound $\gamma_x(s') \le \overline P(s,a)(s')$. Note that, for all $s' \notin C(s,a)$, the interval constraints are not learned: instead, these are implicit and in the form $\gamma_x(s')\in[0,1]$, which are trivially satisfied since $\gamma_x\in\mathcal{P}(S)$. Therefore, the total number of learned intervals for states $s'$ is $\sum_{s\in S, a\in A} |C(s,a)|$. Using again Proposition~\ref{prop:hoeffding} with $\tilde r = \bigcup_{s'\in q'}J^{-1}(s')$ and noting that $T(\tilde r \mid x, a) = \sum_{s'\in q'} T(J^{-1}(s') \mid x, a)$ since the regions in the partition $R$ are disjoint, it follows that $\underline P(s,a)(q') \le \sum_{s'\in q'}\gamma_x(s')$ with confidence $1-\beta/2$ pointwisely for all $q'\in Q(s,a)$, and similarly for the upper bound $\sum_{s'\in q'}\gamma_x(s') \le \overline P(s,a)(q')$. This makes the total number of learned intervals for clusters $q'$ be $\sum_{s\in S, a\in A} |Q(s,a)|$.

    \iffalse
    Furthermore, let $B := \{f(x,w)\in\mathbb{R}^n : w \in\widehat W\}$ and note that, in general, $f^{-1}(B) \supseteq \widehat W$. Then,
    %
    \begin{align*}
        P_W(f^{-1}(B)) \ge P_W(\widehat W) \ge 1-\epsilon_c.
    \end{align*}
    %
    Since, by Lemma... the last inequality holds with
    \fi

    Furthermore, since, by definition, $C(s,a) \supseteq \widehat{\text{Post}}(s,a)$, we also have that
    %
    % \begin{align*}
        % &\sum_{s'\in C(s,a)}\gamma_x(s') \ge \sum_{s'\in \widehat{\text{Post}}(s,a)}\gamma_x(s') = \sum_{s'\in \widehat{\text{Post}}(s,a)}T(J^{-1}(s')\mid x,a)
        % = T(\bigcup_{s'\in \widehat{\text{Post}}(s,a)} J^{-1}(s') \mid x,a)\\
        % &= P(\{w\in W : f(x,a,w) \in \bigcup_{s'\in \widehat{\text{Post}}(s,a)} J^{-1}(s')\}) = P(\{w\in W : J(f(x,a,w)) \in \widehat{\text{Post}}(s,a)\}) \ge P(\widehat W),
    % \end{align*}
    %
    $\sum_{s'\in C(s,a)}\gamma_x(s') \ge$\\ $\sum_{s'\in \widehat{\text{Post}}(s,a)}\gamma_x(s') = \sum_{s'\in \widehat{\text{Post}}(s,a)}T(J^{-1}(s')\mid x,a)
    = T(\bigcup_{s'\in \widehat{\text{Post}}(s,a)} J^{-1}(s') \mid x,a)
    = P_W(\{w\in W : f(x,a,w) \in \bigcup_{s'\in \widehat{\text{Post}}(s,a)} J^{-1}(s')\}) = P_W(\{w\in W : J(f(x,a,w)) \in \widehat{\text{Post}}(s,a)\}) \ge P_W(\widehat W),$
    which is at least $1-\epsilon_c$ with confidence at least $1-\beta_c$. Then, it follows that the last constraint in \eqref{eq:Gamma} also holds with the same confidence. Combining this confidence with the $\sum_{s\in S, a\in A} |C(s,a)| + |Q(s,a)|$ learned intervals via the union bound, we get that $\gamma_x$ fulfills all constraints in the definition at least $\Gamma_{s,a}$ with confidence $1-\alpha$.
\end{proof}
\fi
%
\begin{corollary}
    \label{cor:sample_complexity}
    Given $\alpha \in (0,1)$ and $\epsilon, \epsilon_c \in (0,1)$, the sample complexity of obtaining a UMDP abstraction with confidence at least $1-\alpha$ is
    %\begin{align*}
        $N = \max\big\{\log( \frac{n_\text{learn}/\alpha}{2\epsilon^2}), \log(\frac{n_\text{learn}/\alpha}{\log{(1/(1-\epsilon_c}))}) \big\}$,
    %\end{align*}
    %
    with $n_\text{learn} = 1+ \sum_{s\in S\setminus\{s_{|S|}\}, a\in A} |C(s,a)| + |Q(s,a)|$.
\end{corollary}
%Since $\Gamma_{s,a}$ is non-empty with confidence at least $1-\alpha$, it is easy to verify that the conditions in \eqref{eq:conditions_rmdp} \ml{these conditions are commented out now.  Should we refer to \eqref{eq:data_driven_bounds}? Or say, the bounds in \eqref{eq:Gamma}??} are satisfied with the same confidence. \ig{This is needed for correctness of the algorithm. Put there}


% \input{Sections/naiive_imdp}

% \subsection{Issues of Na\"ive Data-Driven IMDP Abstractions}
% \label{sec:issues}

% \ml{move this section to the supplementary material.}

% % As mentioned above, compared to the abstraction classes frequently used in the literature, namely, interval MDPs (IMDPs) \ig{cite}, our UMDP abstraction differs in that the sets $\Gamma_{s,a}$ of transition probability distributions are defined by more constraints than just the intervals $[\underline P(r_s,a)(r_{s'}), \overline P(r_s,a)(r_{s'})]$ for all $s'\in S$. Here, we discuss why IMDPs are not a good abstraction choice in our setting, and thus why a more complex $\Gamma$ is required.

% As noted earlier, unlike the commonly used abstraction classes in the literature, such as interval MDPs (IMDPs) \ig{cite}, our UMDP abstraction defines the sets $\Gamma_{s,a}$ of transition probability distributions with more constraints than just the intervals $[\underline P(r_s,a)(r_{s'}), \overline P(r_s,a)(r_{s'})]$ for all $s' \in S$. Below, we explain why IMDPs are unsuitable for our setting and why a more complex definition of $\Gamma$ is necessary through an example.
% %
% \begin{example}
%     Let $\mathcal{I}$ be a UMDP abstraction of System~\eqref{eq:sys}, where $\Gamma$ is only represented by the interval bounds $\underline P(r_s,a)(r_{s'}), \overline P(r_s,a)(r_{s'})$ for all $s'\in S$, making $\mathcal{I}$ an interval MDP (IMDP). For simplicity and without loss of generality, consider the reach-avoid specification $\varphi := \Diamond\rm{goal}\land \Box( \neg\rm{unsafe})$. %Consider also that the state-space discretization was obtained uniformly gridding $X$.
%     Note that the event $\text{Reach}(r_s,a,\boldsymbol{\hat w})\subseteq r_{s'}$ present in \eqref{eq:conditions} rarely happens, since it requires that the reachable set is smaller than the region $r_{s'}$. In turn, this event is uncommon in a big portion of the state-space unless the system's dynamics are $1$-step contractive and that the partition is "aligned" with the dynamics. As a consequence, %when $s'$ is not a terminal state, e.g., the goal or unsafe regions, which are typically way bigger than the rest,
%     $\underline P(s,a)(s')$ is very often zero. However, the upper bound $\overline P(s,a)(s')$ behaves very differently: by \eqref{eq:conditions}, $\overline P(s,a)(s') \ge \epsilon$ for all $s'\in S$. %Consider the states $\widehat S := \{s'\in S : \exists i\in\{1,\dots, N\}\:\text{s.t.}\: \text{Reach}(r_s,a,\boldsymbol{\hat w}^{(i)})\bigcap r_{s'} \neq \emptyset\}$, i.e., the set of abstract states $s'$ whose corresponding region $r_{s'}$ intersects the reachable set corresponding to some sample of $\w$, and note that typically $|\widehat S| \ll |S|$. 
    
%     Consider now the strategy synthesis process for a simple reach-avoid specification, which is carried out via robust dynamic programming. At each iteration, denote by $S_k$ the set of states with zero value function, i.e., the goal states, and note that, typically, $|S_k| \approx |S|$ during the first iterations. Denote by $\widehat S_k\subseteq S$ the set of abstract states $s$ such that $\underline P(s,a)(s') = 0$ for all $s'\in S_k$, and note that, in general, $|\widehat S| \approx |S|$. Now, by construction of $\I$, the adversary $\xi$ is allowed to pick a distribution over $S$ that assigns probability $\epsilon$ of transitioning to every $s'\in \widehat S$, and that, if $S$ is big enough, the total probability of transitioning to these states adds up to $1$. Note that refining the abstraction eventually leads to this condition. As a result, the value function at the iteration $k+1$ is again zero for all $s\in\widehat S$. This phenomenon yields a vacuous satisfaction probability on a big region of the state space.
% \end{example}


\section{Strategy Synthesis}
\label{sec:synthesis}

% In this section, we focus on synthesizing a strategy for System~\eqref{eq:sys} and lower-bound the probability that the closed-loop system satisfies the \LTLf specification $\varphi$. 
% %\LTLf formula $\varphi$.
% To that end, we first synthesize a strategy $\sigma\in\Sigma$ for $\M$ that (robustly) maximizes the probability of satisfying $\varphi$, and then refine the obtained strategy into a strategy $\sigma_x$ of System~\eqref{eq:sys} in a way that the satisfaction probability bounds are preserved. 
%
\iffalse

%We begin by showing that strategy synthesis for $\M$ is equivalent to solving a robust maximal reachability problem in an augmented UMDP.
%
\begin{definition}[DFA]
    Let $\varphi$ be an \LTLf formula defined over a set of atomic propositions $AP$. The \emph{deterministic finite automaton} (DFA) corresponding to $\varphi$ is a tuple $\A = (Z,2^{AP},\delta,z_0,Z_F)$ where $Z$ is a finite set of states, $2^{AP}$ is a finite set of input symbols, $\delta:Z\times 2^{AP} \rightarrow Z$ is the transition function, $z_0\in Z$ is the initial state, and $Z_F\subseteq Z$ is the set of accepting states.
\end{definition}

Given a trace $\rho = \rho_0\rho_1 \dots \rho_{K} \in (2^{AP})^*$, a run $z = z_0z_1 \dots z_{K+1}$ is induced on $\A$, where $z_{k+1} = \delta(z_k,\rho_{k})$ for all $k\in \{0,\dots,K\}$. By construction of $\A$, trace $\rho$ satisfies $\varphi$ iff $z_{K+1} \in Z_F$ \cite{de2013linear}. Such a run is called \emph{accepting} for $\A$.

\begin{definition}[Product UMDP]
    Given UMDP $\M$ and DFA $\A$, the product $\PRMDP = \M\otimes\A$ is another UMDP $\PRMDP = (S^\varphi,A^\varphi,\Gamma^\varphi,s_0^\varphi, S_{F}^\varphi)$, where
   $S^\varphi = S\times Z$ %is the set of states
   , $A^\varphi = A$ %is the set of actions
   , $s_0^\varphi = \delta(s_0,L(s_0))$, %is the initial state, 
   $S_F^\varphi = S\times Z_F$ %is the set of accepting states, 
   ,
   and 
    $\Gamma^\varphi = \{\Gamma_{(s,z),a}^\varphi: (s,z)\in S^\varphi, a\in A^\varphi((s,z))\}$ with 
       $
            \Gamma_{(s,z),a}^\varphi := \{\gamma^\varphi \in \mathcal{P}(S^\varphi) : \exists \gamma\in\Gamma_{s,a}\: \text{s.t.}\: \gamma^\varphi((s',z')) = \gamma(s') \: \text{with}\: z' = \delta(z,L(s')), \forall s'\in S\}.
       $
        % \ig{Maybe can be stated in a simpler way: $\Gamma_{(q,z),a}^\varphi$ is the set of distributions over $\{(q',z')\in Q^\varphi : z' = \delta(z,L(q'))\}$ and whose projection on $Q$ yields a distribution $\gamma\in\Gamma_{q,a}$}
\end{definition}

Once obtained the product UMDP, 

\fi
%

% We synthesize $\sigma$ via unbounded-horizon \emph{robust dynamic programming} (RDP) as described in \cite[Theorems 6.2, 6.6]{gracia2025efficient}. This strategy maximizes the probability satisfying $\varphi$ under an adversarial choice of the transition probability distributions from the sets $\Gamma_{s,a}$. %We then refine $\sigma^\varphi$ into a 
% By refining $\sigma$ into $\sigma_x$
%by letting $\sigma_x(\omega_x) = \sigma^\varphi(J(x), z_)$, where $x = \omega_x(|\omega_x|)$ and $z$ is the $|\omega_x|$-th state in the run on $\A$ that is
 % as shown in \ig{cite}, the following guarantees hold:


We now synthesize a strategy for System~\eqref{eq:sys} and lower bound the probability that the closed-loop system satisfies formula $\varphi$. We first show that standard synthesis procedures for general UMDPs from the literature \citep{wolff2012robust,gracia2025efficient}
apply to our setting and introduce a novel (tailored) algorithm that leverages the specific structure of our abstraction for faster computations. 

% The synthesis procedure is as follows. Given the UMDP abstraction $\M$ and an \LTLf specification $\varphi$, first translate $\varphi$ to its equivalent deterministic finite automaton $\A^\varphi$, and then construct product $\M^\varphi = \M \otimes \A^\varphi$.  
% The strategy $\sigma$ is synthesized using unbounded-horizon \emph{robust dynamic programming} (RDP) on $\M^\varphi$ following the approach in \cite[Theorems 6.2, 6.6]{gracia2025efficient}.
% This strategy maximizes the probability of satisfying $\varphi$ under an adversarial choice of the transition probability distributions from the sets $\Gamma_{s,a}$. 
% Then, $\sigma$ is refined into $\sigma_x$, as shown in \ig{cite}.  The following theorem establishes the guarantees of this procedure.
We start by translating $\varphi$ into its equivalent deterministic finite automaton $\A^\varphi$ \citep{de2013linear} and constructing the product $\M^\varphi = \M \otimes \A^\varphi$ \citep{wolff2012robust}. We then synthesize a strategy $\sigma^\varphi$ on $\M^\varphi$ via unbounded-horizon \emph{robust dynamic programming} (RDP) with a reachability objective, as detailed in \cite[Theorems 6.2, 6.6]{gracia2025efficient}. $\sigma^\varphi$ maximizes the probability of satisfying $\varphi$ under adversarial choices of transition probabilities from $\Gamma^\varphi$. Finally, we refine $\sigma^\varphi$ into a strategy $\sigma_x$ for System~\eqref{eq:sys}. Theorem~\ref{thm:strategy_synthesis}, whose proof is given in \cite{supp}, ensures that satisfaction probability bounds are preserved under this procedure, thus solving Problem~\ref{prob:Syntesis}. 
% The following theorem establishes the guarantees of this procedure.

% To synthesizing a strategy for System~\eqref{eq:sys} and lower-bound the probability that the closed-loop system satisfies the \LTLf specification $\varphi$. 
%\LTLf formula $\varphi$.
% To that end, we first synthesize a strategy $\sigma\in\Sigma$ for $\M$ that (robustly) maximizes the probability of satisfying $\varphi$, and then refine the obtained strategy into a strategy $\sigma_x$ of System~\eqref{eq:sys} in a way that the satisfaction probability bounds are preserved. 

\begin{theorem}[Strategy Synthesis through Product UMDP]
\label{thm:strategy_synthesis}
    Let $\sigma^\varphi$ and $\underline p^\varphi$ be respectively the optimal strategy and the lower bound in the probability of satisfying $\varphi$ obtained via RDP on $\M^\varphi$. Denote by $S^\varphi_0$ the set of initial states of $\M^\varphi$ and by $\text{Lift}: S \to S^\varphi_0$ the function that maps states of $\M$ to $S^\varphi_0$. Furthermore, let $\sigma_x$ be the strategy obtained by refining $\sigma^\varphi$ to System~\eqref{eq:sys}. Then, with confidence $1-\alpha$,
    %
    % \begin{align*}
        % Pr_{x}^{\sigma^\varphi}[\pathX \models \varphi \land \Globally \neg \Prop_u] \ge \underline p^\varphi(\text{Lift}(s)),
    % \end{align*}
    %
    $Pr_{x}^{\sigma^\varphi}[\pathX \models \varphi] \ge \underline p^\varphi(\text{Lift}(s))$
    for all $x\in X$, where $s = J(x)$. %, $z = \delta(z_0,L(s))$.
\end{theorem}
%
\iffalse
\begin{proof}
    Assume $\M$ is a correct abstraction of System~\eqref{eq:sys}. Then, it follows that \citep{wolff2012robust} $Pr_{x}^{\sigma^\varphi}[\pathX \models \varphi \land \Globally \neg \Prop_u] \ge \underline p^\varphi(\text{Lift}(s)),$
    for all $x\in X$, where $s = J(x)$. Since by Theorem \ref{theorem:soundness} this assumption holds with confidence $\ge 1-\alpha$, the implication also holds with the same confidence.%, concluding the proof.
\end{proof}
\fi
    %    
\iffalse
\begin{proof}
    We extend the reasoning of \cite{baier2008principles}[p. $882$] to the setting of UMDPs. Note that for every
    path $\path$ of $\M$, with trace $\rho$, the corresponding path $\path^\varphi$ of $\M\otimes\mathcal{A}$ is obtained by letting $\path^\varphi(k) = (s_k,z_k)$, with $z_k = \delta(z_{k-1},L(s_k))$ for all $k$. Reversing the previous argument it follows that there is a $1$-to-$1$ correspondence between the paths of $\M$ and those of $\M\otimes\mathcal{A}$. Moreover, $\path\models\varphi$ if and only if the corresponding $\path^\varphi$ is accepting by $\mathcal{A}$.

    Consider the adversary $\xi\in\Xi$ of $\M$, and let $\gamma_{s,a,k}\in\Gamma_{s,a}$ denote the probability distribution chosen by $\xi$ at state $s\in S$, under action $a\in A$, and at time $k$. Define the adversary $\xi^\varphi$ of $\M\otimes\mathcal{A}$ such that it picks $\gamma_{(s,z),a,k}^\varphi$ at state $s\in S$, under action $a\in A$, and at time $k$, with $\gamma_{(s,z),a,k}^\varphi(s') = \gamma_{(s,z),a,k}((s',z'))$, $z' = \delta(z,L(s'))$, for all $s'\in S$. Note that, by construction, given $\xi$, $\xi^\varphi$ is uniquely defined, and vice-versa.
    Given adversary $\xi$, $\M$, the latter collapses to an MDP with fixed, but time-varying (inhomogeneous) transition probabilities, with probability measure $Pr_s^{\sigma,\xi}$ over its paths. Note that $\sigma^\varphi$ induces a unique strategy $\sigma$  of $\M$, which maps each finite path $\path = s_0\xrightarrow{a_0}s_1\xrightarrow{a_1}\dots\xrightarrow{a_{K-1}} s_K \in \PathFin$ to $\sigma(\path) = \sigma^\varphi((s_K,z_K))$, where $z_K$ is the $K$-th element of the unique run induced by $\path$ on $\mathcal{A}$. Furthermore, for every path $\path$ of $\M$ under $\sigma,\xi$, the corresponding path $\path^\varphi$ exists on $\M\otimes\mathcal{A}$ under $\sigma^\varphi,\xi$. By the total law of probability, we obtain that at time $k$, the probability of transitioning from $(s_k,z_k)$, under action $\sigma^\varphi((s_k,z_k))$, to some state of $\M\otimes\mathcal{A}$ whose first component is $s_{k+1}$ is equal to $\gamma(s_{k+1})$. This implies that the probabilities of the paths $\path$ of $\M$ under $\sigma,\xi$ and the corresponding paths $\path^\varphi$ of $\M\otimes\mathcal{A}$ under $\sigma^\varphi,\xi^\varphi$ is the same. Then, it follows that 
    %
    \begin{align*}
        Pr_{\sigma, \xi}[\path \models \varphi \land \Globally \neg \Prop_u] = Pr_{\sigma^\varphi, \xi^\varphi}[\path^\varphi \models \Diamond S_F^\varphi]
    \end{align*}
    %
    for all adversaries, and therefore the infimum with respect to the adversaries also results in an equality. By... 
    %
    \begin{align*}
        \inf_{\xi^\varphi\in\Xi^\varphi}Pr_{\sigma^\varphi, \xi^\varphi}[\path^\varphi \models \Diamond S_F^\varphi] \le
    \end{align*}
    %
    
    \fi

    \iffalse
    Let $\mathcal{H}$ be the \emph{stochastic hybrid system} with state-space $\reals^n\times Z$ and Borel $\sigma$-algebra $\mathcal{B}(\reals^n\times Z)$ generated by the subsets of $\reals^n\times Z$ of the form $B\times\{z\}$ with $B\in\mathcal{B}(\reals^n)$ and $z\in Z$. The transition kernel $T_\mathcal{H}:\mathcal{B}(\reals^n\times Z)\times (\reals^n\times Z)\times U\rightarrow[0, 1]$ is given by
    %
    %\begin{align*}
        $T(B\times\{z'\} \mid (x, z), u) = 
            T(B\bigcap E(z,z') \mid (x, z), u),$
    %
    where $E(z,z') := \{x'\in\reals^n : \delta(z,L(x')) = z'\}$ and $B\in \mathcal{B}(\reals^n)$, $x \in \reals^n$, $z,z'\in Z$, $u \in U$. By \cite[Theorem 4]{abate2011quantitative}, it holds that the probability of the paths of System~\eqref{eq:sys} satisfying $\varphi$ under strategy $\sigma_x$ and starting at state $x\in r_i$, with $r_i\in R$, is equal to the probability of the paths of $\mathcal{H}$ reaching $S_F$ under strategy $\sigma^\varphi$ and starting at state $(s_i,z_0) \in S\times Z$, with $z_0 = \delta(z_\text{init}, L(s_i))$.

    \ig{WIP... Not sure if we're gonna be able to prove all this within the 10 p. limit}\luca{Is this not basically just the standard correctness result for abstractions to uncertain MDP? Such as Theorem 3 and 4 in \cite{laurenti2023unifying} or in \cite{delimpaltadakis2021abstracting}. If so, just refer to these papers and say the proof follows similarly (maybe you can just mention the differences, if any.)}
    \mm{I'm with Luca. This looks very standard. Maybe worth considering cutting }
    
    Next, we prove that these probabilities are lower bounded by $\underline p(s_i, z_0)$. Note that the latter probability corresponds to the value function $V_{\sigma^\varphi}^{\infty}$ corresponding to the Bellman recursion \cite{abate2011quantitative}
    %
    \begin{align*}
        V_{\sigma^\varphi}^{k+1}(x,z) = \sum_{z'\in Z}\int_{\reals^n} V_{\sigma^\varphi}^{k}(x',z') T((dx'\times\{z'\}) \mid (x, z),\sigma^\varphi(x, z)),
    \end{align*}
    %
    By a similar induction argument as the one in \cite[Theorem 4.1]{delimpaltadakis2021abstracting}
    %
    \begin{align*}
        V_{\sigma^\varphi}^{k+1}(x,z) &= \sum_{z'\in Z}\sum_{i\in\{1,\dots, |S|\}} \int_{r_i} V_{\sigma^\varphi}^{k}(x',z') T((dx'\times\{z'\}) \mid (x, z),\sigma^\varphi(x, z))\\
        &\ge \sum_{z'\in Z}\sum_{i\in\{1,\dots, |S|\}} V_{\sigma^\varphi}^{k}(s_i',z') \int_{r_i}T((dx'\times\{z'\}) \mid (x, z),\sigma^\varphi(x, z))\\
        &\ge \sum_{z'\in Z}\sum_{r_i'\in R} V_{\sigma^\varphi}^{k}(s_i',z') T((r_i'\times\{z'\}) \mid (x, z),\sigma^\varphi(x, z))\\
        &\ge \min_{\gamma^\varphi\in\Gamma^\varphi_{(s,z),\sigma^\varphi(x, z)}}\sum_{(s',z')\in S\times Z}\gamma^\varphi(s',z')V_{\sigma^\varphi}^{k}(s',z') =: V_{\sigma^\varphi}^{k+1}(s,z),\\
    \end{align*}
    %
    where the last inequality follows from the fact that $\gamma^\varphi \in \Gamma^\varphi_{(s,z),\sigma^\varphi(x, z)}$, for $\gamma^\varphi(s_i',z') = T((r_i'\times\{z'\}) \mid (x, z),\sigma^\varphi(x, z))$ This can be seen by the fact that $\gamma^\varphi(s_i', \delta(z,L(s_i'))) = T(r_i' \mid x,a)$ for all $s_i'\in S$, and that by Theorem~\ref{theorem:soundness}, the distribution defined by $\gamma(s_i') := T(r_i' \mid x,a)$ for all $s_i'\in S$ belongs to $\Gamma_{s,a}$.

    Note that, although the previous Bellman recursion corresponds to a fixed strategy $\sigma^\varphi$, the recursion converges to the same probability as recursion... This result follows from the fact that $V^\infty(s,z) = \max_{\sigma\in\Sigma^\varphi} V^\infty_{\sigma}(s,z) = V^\infty_{\sigma^\varphi}(s,z)$.
    %

\end{proof}
\fi

\paragraph{Tailored Synthesis Algorithm}

% Here, we introduce an algorithm to efficiently compute the choice of the adversary in RDP. We highlight that the construction of product $\M^\varphi$ preserves the unique structure of our UMDP $\M$ as shown in the supplementary material \ml{CITE}. In consequence, here we describe how our proposed algorithm works in the simpler setting of a reachability problem on $\M$, instead of on $\M^\varphi$.
\begin{algorithm}[t]\small
 \caption{$2$-layer $O$-maximization}\label{alg:2O}
 \vspace{-4mm}
\begin{multicols}{2}
\begin{algorithmic}[1]
    \Require $\M,s\in S\setminus\{s_{|S|}\}, a\in A, \underline p^k$
    \Ensure $\gamma$
    % \textbf{Input:} $\M,s\in S, a\in A, \underline p^k$, \textbf{Output:} $\gamma$
    \State Sort $\text{Post}(s,a)$ according to $\{\underline p^k(s')\}_{s'\in \text{Post}(s,a)}$ in increasing order
    \State $\gamma(s') \gets \underline P(s,a)(s')$ for all $s'\in \text{Post}(s,a)$
    \State $\gamma(s') \gets 0$ for all $s'\notin \text{Post}(s,a)$
    \State $\gamma(q') \gets \sum_{s'\in q'} \gamma(s')$ for all $q'\in Q(s,a)$
    \State $M \gets 1 - \sum_{s'\in S} \gamma(s')$
    \For{$q'\in Q(s,a)$}
        \State $m \gets \underline P(s,a)(q') - \gamma(q')$
        \If{$m >0$}
            \For{$s'\in q'$}
                \State $g \gets \min\{m, \overline P(s,a)(s') - \gamma(s')\}$
                \State $\gamma(s') \gets \gamma(s') + g$, $\gamma(q') \gets \gamma(q') + g$
                % \State $\gamma(q') \gets \gamma(q') + g$
                \State $m \gets m - g$, $M \gets M - g$
                % \State $M \gets M - g$
                %\If{$m == 0$}
                %    \State \textbf{break}
                %\EndIf
            \EndFor
        \EndIf
    \EndFor
    \iffalse
    %\State $M \gets M - \sum_{q'\in Q} \gamma(q')$
    \For{$q'\in Q$}
    \State $M \gets M - \gamma(q')$
    \For{$s'\in q'\bigcup \text{Post}(s,a)$}
    \State $\gamma(s') \gets \min\{\gamma(q'), \overline P(s,a)(s')\}$
    \State $\gamma(q') \gets \gamma(q') - \gamma(s')$
    \If{$\gamma(q') == 0$}
    \State \textbf{break}
    \EndIf
    \EndFor
    \EndFor
    \fi
    %\State $\gamma(q') \gets \underline P(s,a)(q')$ for all $q'\in Q$
    \For{$s'\in \text{Post}(s,a)$}
    \State $q' \gets$ get cluster $q'$ such that $s'\in q'$
    \If{$q' \neq \emptyset$}
    %\State $b \gets \min\{\overline P(s,a)(q') - \gamma(q'), \overline P(s,a)(s') - \gamma(s')\}$
    \State $m \gets \min\{M, \overline P(s,a)(q') - \gamma(q'),$ $ \qquad \overline P(s,a)(s') - \gamma(s')\}$
    \State $\gamma(q') \gets \gamma(q') + m$
    \Else
    \State $m \gets \min\{M, \overline P(s,a)(s') - \gamma(s')\}$
    \EndIf
    \State $\gamma(s') \gets \gamma(s') + m$, $M \gets M - m$
    % \State $M \gets M - m$
    %\If{$M == 0$}
    %\State \textbf{break}
    %\EndIf
    \EndFor
    %\State $\underline p^{k+1}(s) = \sum_{s'\in S}\gamma(s')\underline p^k(s')$
\end{algorithmic}
\end{multicols}
\vspace{-4mm}
\end{algorithm}


We introduce a synthesis algorithm tailored for UMDPs as such in Definition~\ref{def:umdp abstraction}, which exploits their structure for greater efficiency.  The algorithm 
draws inspirations from IMDP value iteration \citep{givan2000bounded} to speed up the computation of the optimal adversaries in RDP, which is typically formulated a linear program in standard UMDPs. We note that this approach is applicable to our product UMDP $\M^\varphi$ because it retains the same structure of $\M$, as detailed in the supplementary material \cite{supp}. Therefore and, for simplicity, we describe the algorithm in the context of a reachability problem on $\M$ rather than on $\M^\varphi$.   

% Note that, since $\M^\varphi$ has a different structure than the UMDPs considered in \cite{gracia2025efficient}, a different tailored algorithm is required. 

% First note that, for all $s\in S$, $a\in A$, it is possible to simplify the sets $\Gamma_{s,a}$ of $\M$ by discarding the last constraint in \eqref{eq:Gamma}, and then modifying the upper bounds in the transition probabilities accordingly. More formally, we increase $\overline P(s,a)(s_{|S|})$ and $\overline P(s,a)(q')$, for all $q'\in Q(s,a)$ with $s_{|S|}\in q'$, by $\epsilon_c$, and set $\overline P(s,a)(s')=0$ for all $s'\in C(s,a)\setminus \{s_{|S|}\}$ and $\overline P(s,a)(q')=0$, for all $q'\in Q(s,a)$ with $s_{|S|}\notin q'$. In consequence, the adversary is allowed to pick a distribution with a higher probability of transitioning to the unsafe region. It is then easy to check that the solution $\underline p$ obtained via RDP in this new UMDP is not higher than the one obtained for $\M$. 
% We omit the proof 
% \ml{should we refer to the supplementary material instead???}
% for the sake of space, and from now on we assume that $\M$ has been simplified as explained here.

The algorithm first streamlines the uncertainty set of $\M$.
Observe that %for all $s \in S$ and $a \in A$,
the sets $\Gamma_{s,a}$ of $\M$ can be simplified by discarding the last constraint in \eqref{eq:Gamma} and adjusting the transition probability upper bounds accordingly. Specifically, we increase $\overline{P}(r_s,a)(r_{s_{|S|}})$ and $\overline{P}(r_s,a)(r_{q'})$ for all $q' \in Q(s,a)$ with $s_{|S|} \in q'$ by $\epsilon_c$, and set $\overline{P}(r_s,a)(r_{s'}) = 0$ for all $s' \notin C(s,a) \cup \{s_{|S|}\}$. % and $\overline{P}(r_s,a)(r_{q'}) = 0$ for all $q' \in Q(s,a)$ with $s_{|S|} \notin q'$. 
As a result, the adversary can choose a distribution with a higher probability of transitioning to the unsafe region. It can be shown that the solution $\underline{p}$ obtained via RDP in this simplified UMDP is not greater than the one obtained for $\M$. We provide a formal proof in~\citep{supp}, and hereby assume that $\M$ is simplified as described.
\iffalse

\begin{lemma}
    Consider the UMDP $\underline{\mathcal{I}}$ with transition probability intervals
    %
    \begin{align*}
        \underline{P}(s,a)(s') &= \begin{cases}
            CI \:\quad &\forall s' \in C(s,a)\\
            0  \:\quad &\forall s' \notin C(s,a)
        \end{cases} 
        %
        \\
        \overline{P}(s,a)(s') &= \begin{cases}
            CI \:\quad &\forall s' \in C(s,a)\setminus s_{|S|}\\
            0  \:\quad &\forall s' \notin C(s,a)\setminus s_{|S|}\\
            CI + \epsilon_c  \: \quad &\text{if}\: s' = s_{|S|}\:\text{and}\:s' \in C(s,a)\\
            \epsilon_c  \: \quad &\text{if}\: s' = s_{|S|}\:\text{and}\:s' \notin C(s,a)\\
        \end{cases} 
        %
        \\
        \underline{P}(s,a)(q') &= CI \:\:\text{if}\:\:q' \in Q(s,a)\\
        \overline{P}(s,a)(q') &= \begin{cases}
            CI  \: \quad &\text{if}\:q' \in Q(s,a)\:\text{and}\:\: s_{|S|} \notin q'\\
            CI + \epsilon_c  \: \quad &\text{if}\:q' \in Q(s,a)\:\text{and}\:\: s_{|S|} \in q'\\
        \end{cases} 
        %
    \end{align*}
    %
    for all $s\in S$, $a\in A$. We denote $\mathcal{I}$ as \emph{sparse} UMDP. Let $\underbar p$ and $\underbar p^R$ be the lower value functions returned by $\mathcal{A}(\underline{\mathcal{I}}, \varphi)$ and $\mathcal{A}(\M, \varphi)$, respectively. Then, $\underbar p(s) \le \underbar  p^R(s)$ for all $s\in S$.
    \end{lemma}
    %
    \begin{proof}
        Let $V^k$ denote the $k$-th iteration of robust dynamic programming. Consider $s\in S$ and $a\in A$.
        %
        \begin{align*}
            \min_{\gamma\in\Gamma_{s,a}}\sum_{s'\in S}\gamma(s') p^k(s')
        \end{align*}
        %
        Note that a minimizer $\Gamma\in\Gamma_{s,a}$ of the previous problem is any $\Gamma$ that assigns as much probability mass as possible to the states $s'\in S$ with the smallest $p^k(s')$. Note that, by the last constraint in the definition of $\Gamma_{s,a}$, at least $1-\epsilon_c$ mass must be allocated to the states in $C(s,a)$. Define $\gamma^l(s') := \Gamma(s')$ for all $s'\in C(s,a)\setminus\{s_{|S|}\}$, $\gamma^l(s_{|S|}) := \Gamma(s_{|S|}) + \epsilon_c$ and $\gamma^l(s') := 0$ everywhere else. Then, it is easy to observe that $\gamma^l\in\Gamma^l_{s,a}$. Furthermore, $\sum_{s'\in S}\Gamma(s') p^k(s')  = \sum_{s'\in S}\gamma^l(s') p^k(s')$, thus implying that
        %
        \begin{align*}
            \min_{\gamma\in\Gamma_{s,a}}\sum_{s'\in S}\Gamma(s') p^k(s') = \sum_{s'\in S}\Gamma(s') p^k(s')  = \sum_{s'\in S}\gamma^l(s') p^k(s') \ge \min_{\gamma\in\Gamma^l_{s,a}}\sum_{s'\in S}\gamma(s') p^k(s')
        \end{align*}
        %
        Maximizing over the actions on both sides yields $p_\M^{k+1}(s) \le p_l^{k+1}(s)$ for all $s\in S$.
        Using this result in an induction argument and letting $k\to\infty$ concludes the proof.
    \end{proof}

    \fi
%\ml{this seems out of place.  Please fix it.} It is easy to verify that $\Gamma^\varphi$ possesses the same structure as $\Gamma$, thus allowing to perform strategy synthesis via Algorithm~\ref{alg:2O}. 
Then, on the modified $\M$, Alg.~\ref{alg:2O} computes the optimal adversary for each state-action pair $(s,a)$ by extending the O-maximizing algorithm devised for IMDP value iteration \citep{givan2000bounded} to $\M$:  
via a 2-layer O-maximizing logic,
the algorithm efficiently allocates probability mass to states of $\M$ with the lowest value function while respecting the constraints in \eqref{eq:Gamma}. 
It begins by ensuring that the lower bounds $\underline P(r_s,a)(r_{s'})$ are satisfied for all states $s'$ (Lines 2-3), then proceeds to allocate mass to each cluster $q'\in Q(s,a)$ to meet the required lower bounds (Lines 4-12). The algorithm ensures that the total probability mass remains feasible by maintaining the constraints $\gamma(s') \le \overline P(r_s,a)(r_{s'})$, $\sum_{s'\in q'}\gamma(s') \le \overline P(r_s,a)(r_{q'})$ throughout the allocation (Lines 13-20). This allocation process guarantees that as much mass as possible is assigned to states with the smallest value function while ensuring $\gamma \in\Gamma_{s,a}$. Alg.~\ref{alg:2O} terminates once all mass is allocated.%, ensuring the resulting distribution $\gamma$ belongs to the feasible set $\Gamma_{s,a}$, while minimizing the reachability probability objective.  
Note that RDP algorithm \citep{gracia2025efficient} calls Alg.~\ref{alg:2O} for every $(s,a)$ and in every iteration until termination.  The following theorem proves its correctness and runtime complexity.

%
\iffalse
\begin{proposition}
\label{prop:product_bounds}
    For each $(s,z)\in S^\varphi$, $a\in A^\varphi$, $q'\in Q(s,a)$, let $q'^\varphi := \{(s',z')\in q'\times Z : z' = \delta(z, L(s'))\}$, and define $Q^\varphi(s,a)$ as the set of all these $q'^\varphi$. Denote also by $\text{Proj}_S: S^\varphi \rightarrow S$ the projection operator onto $S$. Then, $\Gamma^\varphi_{(s,z),a}$ can be expressed in the form of \eqref{eq:Gamma}, with $\underline{P}((s,z),a)((s',z')) :=
            \underline{P}(s,a)(s')$, $\overline{P}((s,z),a)((s',z')) :=
            \overline{P}(s,a)(s')$ if $z' = \delta(z,L(s'))$ and $0$ otherwise, and $\underline{P}((s,z),a)(q'^\varphi) :=
            \underline{P}(s,a)(\text{Proj}_S(q'^\varphi))$, $\overline{P}((s,z),a)(q'^\varphi) :=
            \overline{P}(s,a)(\text{Proj}_S(q'^\varphi))$
    %
    \iffalse
    
    \begin{align*}
    \begin{split}
        \underline{P}((s,z),a)((s',z')) &:= \begin{cases}
            \underline{P}(s,a)(s')\quad &\text{if}\:\:z' = \delta(z,L(s')),\\
            0\quad &\text{otherwise}
        \end{cases}\\ 
        \overline{P}((s,z),a)((s',z')) &:= \begin{cases}
            \overline{P}(s,a)(s')\quad &\text{if}\:z' = \delta(z,L(s')),\\
            0\quad &\text{otherwise}
        \end{cases}\\
    \end{split}
    \end{align*}
%
and
%
    \begin{align*}
    \begin{split}
        \underline{P}((s,z),a)(q'^\varphi) &:=
            \underline{P}(s,a)(\text{Proj}_S(q'^\varphi))\\ 
        \overline{P}((s,z),a)(q'^\varphi) &:= \overline{P}(s,a)(\text{Proj}_S(q'^\varphi))
\end{split}
\end{align*}

\fi
%
for all $q'^\varphi \in Q^\varphi((s,z),a)$.
%
\end{proposition}
%
\begin{proof}
    Pick an arbitrary $(s, z)\in S^\varphi$ and $\gamma^\varphi\in\mathcal{P}(S^\varphi)$ that satisfies the bounds in Proposition~\ref{prop:product_bounds}. By the interval bounds for each $(s',z')\in S^\varphi$, we have that $\gamma^\varphi((s', z')) = 0$ for all $z' \neq \delta(z, L(s'))$. Define $\gamma\in\mathcal{P}(S)$ as $\gamma(s') := \gamma^\varphi(s', \delta(z,L(s')))$ for all $s'\in S$.  Note that $\gamma$ is a probability over $S$ because $\sum_{s'\in S}\gamma(s') = \sum_{s'\in S}\gamma^\varphi((s',\delta(z, L(s')))) = \sum_{(s',z')\in S^\varphi}\gamma^\varphi((s',z')) = 1$. Since, for each $(s',z')\in S^\varphi$, $\gamma^\varphi((s',z'))\in[\underline{P}((s,z),a)((s',z')), \overline{P}((s,z),a)((s',z'))]$, it is easy to see that $\gamma(s')\in[\underline{P}(s,a)(s'), \overline{P}(s,a)(s')]$ for all $s'\in S$. Next, pick $q'\in Q(s,a)$ and let $q'^\varphi$ be the corresponding set in $Q^\varphi((s,z),a)$. Since $q' = \text{Proj}_S(q'^\varphi)$ we obtain $\sum_{s'\in q'} \gamma(s') = \sum_{s'\in q'} \gamma^\varphi((s', \delta(z, L(s'))) = \sum_{(s',z')\in q'^\varphi} \gamma^\varphi((s',z'))\in[\underline{P}((s,z),a)(q'^\varphi), \overline{P}((s,z),a)(q'^\varphi)] = [\underline{P}((s,z),a)(q'), \overline{P}((s,z),a)(q')]$, which concludes the proof.
\end{proof}
\fi

% \iffalse
% \subsection{Algorithm}
% \label{sec:algorithm}

% \begin{wrapfigure}{L}{0.5\textwidth}
% \begin{minipage}{.5\textwidth}
% \end{minipage}
% \end{wrapfigure}
% \fi

% \input{Sections/alg}

\begin{theorem}[Correctness of Algorithm~\ref{alg:2O}]
\label{thm:soundness_alg}
    Let $k\in\naturals\cup\{0\}$, $s\in S\setminus\{s_{|S|}\}$, $a\in A$ and $\underline p^k\in\reals^{|S|}$ be the value function obtained after $k$ iterations of RDP. Define $\text{Post}(s,a) := \{s' \in S : \overline P(r_s,a)(r_{s'}) > 0\}$. Then, the output $\gamma$ of Algorithm~\ref{alg:2O} satisfies $\gamma \in \arg\min_{\gamma\in\Gamma_{s,a}}\sum_{s'\in S}\gamma(s') \underline p^k(s')$, and it has a computational complexity of $\mathcal{O}(|\text{Post}(s,a)|\log(|\text{Post}(s,a)|))$.
\end{theorem}
%
The proof of Theorem~\ref{thm:soundness_alg} is provided in \citep{supp}. Note that the computational complexity of solving the linear program in the theorem statement using a standard Simplex algorithm is of $\mathcal{O}(|\text{Post}(s,a)|^3)$, highlighting the computational advantage of using Alg.~\ref{alg:2O}.

\begin{remark}
    Note that classical IMDP abstractions use only the first constraint of $\Gamma$ in \eqref{eq:Gamma}, giving the adversary freedom to choose worse $\gamma$ than if the abstraction were like our UMDPs. Consequently, IMDPs yield lower probabilistic guarantees, further motivating our abstraction choice.
\end{remark}


%
\iffalse
\begin{proof}
    We equivalently prove that any $\gamma$ generated by the algorithm belongs to $\Gamma_{s,a}$, and that $\gamma$ assigns the most probability to states $s'\in \text{Post}(s,a)$ with the smallest $\underline p^k(s')$. First we prove that $\gamma\in\Gamma_{s,a}$. From lines $2$ and $3$, we know that $\gamma(s') \ge \underline P(s,a)(s')$ for all $s'\in S$. Furthermore, by construction of $\M$, it is easy to verify that $\underline P(s,a)(q') \le \sum_{s'\in q'}\underline P(s,a)(s')$ for all, $q'\in Q(s,a)$, and therefore lines $4-14$ guarantee that each $q'\in Q(s,a)$ receives exactly $\underline P(s,a)(q')$ probability mass. Since, also by construction, $\gamma(q') \ge \underline P(s,a)(q')$ and that $\underline P(s,a)(q') \le \sum_{s'\in q'}\overline P(s,a)(s')$ for all $q'$, this allocation of probability mass is always feasible, and line $15$ is reached with $m=0$. Additionally, by the logic of lines $10-11$, $\gamma(s') \le \overline P(s,a)(s')$ for all $s'$ so far. %Note that, since $\underline P(s,a)(q') \le \sum_{s'\in q'\bigcap\text{Post}(s,a)} \overline P(s,a)(s')$ by definition \ig{maybe explain a bit more}, this allocation is always feasible, and line $20$ is always reached with $m=0$.
     In lines $15-24$ we allocate the remaining mass from $M$ to the states $s'\in \text{Post}(s,a)$ while respecting $\gamma(s') \le \overline P(s,a)(s')$ and $\gamma(q') \le \overline P(s,a)(q')$. Since $\Gamma_{s,a}\neq\emptyset$, $\sum_{s'\in \text{Post}(s,a)} \overline P(s,a)(s') \ge 1$% and $\sum_{q'\in Q(s,a)} \overline P(s,a)(q') \ge 1$
     , line $24$ is reached with $M=0$. Furthermore, by construction of $\M$, the constraint $\gamma(q') \le \overline P(s,a)(q')$ never prevents all mass from $M$ to be allocated. Therefore, $\gamma\in\Gamma_{s,a}$. %Additionally, the algorithm terminates in finite time. 
     Furthermore, since 1) the algorithm assigns first the least amount of mass that guarantees satisfaction of the lower bounds $\underline P(s,a)(s'), \underline P(s,a)(q')$ for all $s',q'$, 2) when mass is assigned to $\gamma(s')$ (lines $2,3,11,23$), the states with smaller $\underline p^k(s')$ are considered first, and 3) the mass allocated to such states is the maximum amount that the upper bounds $\overline P(s,a)(s'), \overline P(s,a)(q')$ allow. It follows that $\gamma$ minimizes the expression in Theorem~\ref{thm:soundness_alg}. Finally we prove the statement regarding the computational complexity. Note that the for loops in lines $15$ and $17$ are not nested. Additionally, since the sets $q'\in Q(s,a)$ are disjoint, the for loops in lines $6$ and $9$ are equivalent to a single for loop on $s'\in S$. Therefore lines $2$ through $23$ have complexity $\mathcal{O}(|\text{Post}(s,a)|)$, which is negligible in comparison with the complexity of sorting in line $1$, which is $\mathcal{O}(|\text{Post}(s,a)|\log(|\text{Post}(s,a)|))$. Therefore the algorithm has complexity $\mathcal{O}(|\text{Post}(s,a)|\log(|\text{Post}(s,a)|))$, which concludes the proof.
\end{proof}
%
\fi





\iffalse 

\section{Old Stuff}

\subsection{UMDP Abstraction}

Let $\widehat{\text{Post}}(s,a)$ denote the set of states of the abstraction that correspond to the reachable set of region $r \in R(s)$ under action $a$ and for all disturbances $w\in \widehat W$, namely, $\widehat{\text{Post}}(s,a) := \{s' \in S : R(s') \bigcap \text{Reach}(\text{cl}(R(s)),a,\widehat W) \neq \emptyset\}$.

The set $\{\Gamma_{s,a}^R\}_{s\in S, a\in A}$ of transition probability distributions of the UMDP is
%
\begin{align*}
    \Gamma_{s,a}^R := \{\gamma \in \mathcal{D}(S) : \underline{P}(s,a)(s') \le \gamma(s') \le \overline{P}(s,a)(s') \:\forall s' \in \widehat{\text{Post}}(s,a), \sum_{s'\in \widehat{\text{Post}}(s,a)}\gamma(s') \ge 1 - \epsilon_c\}
\end{align*}
%

\begin{lemma}[Soundness of UMDP Abstraction]
    For all $s\in S$, $a\in A$, $x\in r = R(s)$, define $\gamma_x\in\mathcal{P}(S)$ as
    %
    \begin{align*}
        \gamma_x(s') := T(R(s')\mid x,a) 
    \end{align*}
    %
    for all $s'\in S$. Then, $\gamma_x\in \Gamma_{s,a}$ for all $s\in S$, $a\in A$, $x\in r = R(s)$  with confidence $1-\alpha$, $\alpha = \beta_c + \bigg( \sum_{s\in S, a\in A} |\widehat{\text{Post}}(s,a)| \bigg)\beta$.
\end{lemma}
%
\begin{proof}
    From Lemma... we have that $\underline P(s,a)(s') \le \gamma(s')$ with confidence $1-\beta/2$ pointwisely for all $s'\in \widehat{\text{Post}}(s,a)$, and similarly for the lower bound $\gamma(s') \le \overline P(s,a)(s')$. Note that all $s' \notin \widehat{\text{Post}}(s,a)$ are not constrained to lie on learned intervals, so the total number of learned intervals is $\sum_{s\in S, a\in A} |\widehat{\text{Post}}(s,a)|$. Furthermore, let $B := \{f(x,w)\in\mathbb{R}^n : w \in\widehat W\}$ and note that, in general, $f^{-1}(B) \supseteq \widehat W$. Then,
    %
    \begin{align*}
        P_W(f^{-1}(B)) \ge P_W(\widehat W) \ge 1-\epsilon_c.
    \end{align*}
    %
    Since, by Lemma... the last inequality holds with
    %
    \begin{align*}
        \sum_{s'\in \widehat{\text{Post}}(s,a)}\gamma(s') = \sum_{s'\in \widehat{\text{Post}}(s,a)}T(R(s')\mid x,a)\\
        = T(\bigcup_{s'\in \widehat{\text{Post}}(s,a)}R(s') \mid x,a) = P(\{w\in W : f(x,a,w) \in \bigcup_{s'\in \widehat{\text{Post}}(s,a)}R(s')\})
    \end{align*}
    %
    Since, by definition of $\widehat{\text{Post}}(s,a)$ we have that $\bigcup_{s'\in \widehat{\text{Post}}(s,a)}R(s') \supseteq \text{Reach}(\text{cl}(R(s)),a,\widehat W)$, then
    %
    \begin{align*}
        P_W(\{w\in W : f(x,a,w) \in \bigcup_{s'\in \widehat{\text{Post}}(s,a)}R(s')\}) &\ge P_W(\{w\in W : f(x,a,w) \in \text{Reach}(\text{cl}(R(s)),a,\widehat W)\}) \ge P_W(\widehat W) \ge 1-\epsilon_c.
    \end{align*}
    %
     Since the last inequality holds with confidence greater than $1-\beta_c$, it follows that the last constraint in the definition of $\Gamma_{s,a}$ holds also with the same confidence. Combining the confidences over the learned $\widehat W$ and the $\sum_{s\in S, a\in A} |\widehat{\text{Post}}(s,a)|$ learned intervals via the union bound, we get that $\gamma_x$ fulfills all constraints in the definition of $\Gamma_{s,a}$ with overall confidence $1-\beta_c - \bigg( \sum_{s\in S, a\in A} |\widehat{\text{Post}}(s,a)| \bigg)\beta$
\end{proof}



\subsection{Strategy Synthesis via Interval Value Iteration}

\begin{lemma}
    Consider the IMDP $\underline{\mathcal{I}}$ with transition probability intervals
    %
    \begin{align*}
        \underline{P}(s,a)(s') &= \begin{cases}
            CI \:\quad &\forall s' \in \widehat{\text{Post}}(s,a)\\
            0  \:\quad &\forall s' \notin \widehat{\text{Post}}(s,a)
        \end{cases} 
        %
        \\
        \overline{P}(s,a)(s') &= \begin{cases}
            CI \:\quad &\forall s' \in \widehat{\text{Post}}(s,a)\setminus s_{|S|}\\
            0  \:\quad &\forall s' \notin \widehat{\text{Post}}(s,a)\setminus s_{|S|}\\
            CI + \epsilon_c  \: \quad &\text{if}\: s' = s_{|S|}\:\text{and}\:s' \in \widehat{\text{Post}}(s,a)\\
            \epsilon_c  \: \quad &\text{if}\: s' = s_{|S|}\:\text{and}\:s' \notin \widehat{\text{Post}}(s,a)\\
        \end{cases} 
        %
    \end{align*}
    %
    for all $s\in S$, $a\in A$. Let $\underbar p$ and $\underbar p^R$ be the lower value functions returned by $\mathcal{A}(\underline{\mathcal{I}}, \varphi)$ and $\mathcal{A}(\M, \varphi)$, respectively. Then, $\underbar p(s) \le \underbar  p^R(s)$ for all $s\in S$.
    %
    \begin{proof}
        Let $V^k$ denote the $k$-th iteration of robust dynamic programming. Consider $s\in S$ and $a\in A$.
        %
        \begin{align*}
            \min_{\gamma\in\Gamma_{s,a}}\sum_{s'\in S}\gamma(s') p^k(s')
        \end{align*}
        %
        It is known (CITE GIVAN'S PAPER) that a minimizer $\Gamma\in\Gamma_{s,a}$ of the previous problem is any $\gamma$ assigns as much probability mass as possible to the states $s'\in S$ with the smallest $p^k(s')$. Note that, by the last constraint in the definition of $\Gamma_{s,a}$, at least $1-\epsilon_c$ mass is allocated to the states in $\widehat{\text{Post}}(s,a)$. Define $\gamma^l(s') := \Gamma(s')$ for all $s'\in\widehat{\text{Post}}(s,a)\setminus\{s_{|S|}\}$, $\gamma^l(s_{|S|}) := \Gamma(s_{|S|}) + \epsilon_c$ and $\gamma^l(s') := 0$ everywhere else. It is easy to observe then that $\gamma^l\in\Gamma^l_{s,a}$. Furthermore, $\sum_{s'\in S}\Gamma(s') p^k(s')  = \sum_{s'\in S}\gamma^l(s') p^k(s')$, thus implying that
        %
        \begin{align*}
            \min_{\gamma\in\Gamma_{s,a}}\sum_{s'\in S}\Gamma(s') p^k(s') = \sum_{s'\in S}\Gamma(s') p^k(s')  = \sum_{s'\in S}\gamma^l(s') p^k(s') \ge \min_{\gamma\in\Gamma^l_{s,a}}\sum_{s'\in S}\gamma(s') p^k(s')
        \end{align*}
        %
        Maximizing over the actions on both sides yields $p_\M^{k+1}(s) \le p_l^{k+1}(s)$ for all $s\in S$.
        Using this result in an induction argument concludes the proof.
    \end{proof}
    \iffalse
%
\begin{align*}
    \inf_{\xi\in\Xi}Pr_\mathcal{I}[\omega \models \varphi : \omega(0) = s_0, \sigma, \xi] \le \inf_{\xi\in\Xi}Pr_\M[\omega \models \varphi : \omega(0) = s_0, \sigma, \xi]
\end{align*}
%
\fi
\end{lemma}

\begin{lemma}
    Consider the IMDP $\overline{\mathcal{I}}$ with transition probability intervals
    %
    \begin{align*}
        \underline{P}(s,a)(s'), \overline{P}(s,a)(s') = \dots \:\forall s' \in \widehat{\text{Post}}(s,a)\\
        \underline{P}(s,a)(s^*), \overline{P}(s,a)(s^*) = \epsilon_c
    \end{align*}
    %
    for all $s\in S$, $a = \sigma^*(s)$, and where $s^*$ is some state with $\overline{V}(s^*) = 1$. Let $\bar p$ and $\bar p^R$ be the upper
    value functions returned by $\mathcal{A}(\overline{\mathcal{I}}, \varphi)$ and $\mathcal{A}(\M, \varphi)$, respectively. Then, $\bar p(s) \le \bar  p^R(s)$ for all $s\in S$.
\end{lemma}


\fi





==> Sections/5_case_studies.tex <==
\section{Case Studies}
\label{sec:case_studies}

We now demonstrate empirically the effectiveness of our approach through $7$ case studies. These include a nonlinear pendulum with non-additive %under an aerodynamic drag 
disturbances, kinematic unicycle models with $2$- and $3$-D state-spaces and under nonlinear coulomb friction, a $2$-D linear system with multiplicative noise, and a $4$-D thermal regulation benchmark with multiplicative uncertainty. The considered specifications are reach-avoid ($\varphi_1$), the \LTLf specification from \citep{gracia2024data} ($\varphi_2$) and a $15$-step safety specification ($\varphi_3$). For details of these %systems, specifications, and case study 
setups, see \citep{supp}.

\begin{table}[t]
    \centering
    \caption{\small
    % Benchmark results. In ``Approach'' we indicate what is the abstraction we used: UMDP denotes an abstraction as in Definition~\ref{def:robust_mdp}, ``IMDP (Learn Support)'' refers to a UMDP having only the first and third constraints in \eqref{eq:Gamma}, and ``Na\"ive IMDP'' denotes a traditional IMDP abstraction. $e_{avg}$ denotes the average difference (over all states) between the lower and upper bounds in the satisfaction probabilities. The time required for abstraction and synthesis are given in minutes. %, for which respective timeouts of $8$ and $2$ hours are fixed.
    % We denote the number of samples of the noise after clustering by $N_\text{cluster}$.
    Benchmark results. ``Approach" indicates the abstraction used: UMDP (Definition~\ref{def:robust_mdp}), ``IMDP (Learn Support)" (a UMDP with only the first and third constraints in \eqref{eq:Gamma}), and ``Na\"ive IMDP" (traditional IMDP). $e_{avg}$ denotes the average difference in satisfaction probabilities between the lower and upper bounds across all states. Time for abstraction and synthesis is given in minutes, and $ N_\text{cluster}$ denotes the number of noise samples after clustering. The confidence in all case studies is $1-\alpha = 1-10^{-9}$ and $\beta_c = \alpha/2$.
    }
    \scalebox{0.66}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        System (Spec.) & Approach & $|Q|$ & $|A|$ & $N$ & $N_\text{cluster}$ & $e_{avg}$ & Abstr. Time & Synth. Time \\
        \midrule
        Pendulum ($\varphi_1$) & UMDP & $10^4$ & $5$ & $5\times 10^3$ & $47$ & $0.552$ & $1.796$ & $3.643$ \\
        \cite{gracia2024data} & UMDP & $10^4$ & $5$ & $10^4$ & $44$ & $0.007$ & $1.857$ & $6.679$ \\
        & UMDP & $10^4$ & $5$ & $10^5$ & $47$ & $0.003$ & $1.797$ & $2.515$ \\
        %& UMDP & $4\times10^4$ & $5$ & $10^{6}$ & $47$ & $0$ & $7.915$ & $84.539$ \\
        & \cite{gracia2024data} & $4\times10^4$ & $5$ & $10^{6}$ & $49$ & $0$ & $5.273$  & $61.167$ \\
         %&  &  &  & $0.018$ & $-$ & $-$ & $-$ & timeout & $-$ \\
        \midrule
        Pendulum ($\varphi_1$) & UMDP & $1.225\times 10^5$ & $5$ & $5\times10^4$ & $172$ & $0.108$ & $130.680$ & $203.817$ \\
        %(Torque-Limited)& UMDP & $6.25\times 10^4$ & $5$ & $10^5$ & $175$ & $0.082$ & $40.602$ & $70.773$ \\
        (Torque-Limited) & UMDP & $4\times 10^4$ & $5$ & $5\times10^4$ & $173$ & $0.440$ & $31.328$ & $15.203$ \\
        & UMDP & $4\times 10^4$ & $5$ & $10^5$ & $179$ & $0.186$ & $30.952$ & $40.241$ \\
        & UMDP & $4\times 10^4$ & $5$ & $10^6$ & $179$ & $0.048$ & $30.626$ & $29.936$ \\
        & UMDP & $4\times 10^4$ & $5$ & $10^7$ & $191$ &  $0.033$ & $40.520$ & $25.308$ \\
        & IMDP (Learn Support) & $4\times 10^4$ & $5$ & $10^7$ & $191$ &  $0.164$ & $16.714$ & $29.119$ \\
        \midrule
        $3D$ Unicycle ($\varphi_1$) & UMDP & $5.932\times10^4$ & $10$ & $10^{4}$ & $235$ & $0.579$ & $34.689$ & $33.156$ \\
        \cite{gracia2024data} & UMDP & $5.932\times10^4$ & $10$ & $10^{5}$ & $325$ & $0.267$ & $45.610$ & $36.18$ \\
        & UMDP & $5.932\times10^4$ & $10$ & $10^{6}$ & $358$ & $0.156$ & $52.733$ & $33.751$ \\
        & \cite{gracia2024data} & $6.4\times10^4$ & $10$ & $5\times10^{8}$ & $8869$ & $0.447$ & $457.431$ & $43.342$\\
        \midrule
        $3D$ Unicycle ($\varphi_1$) & UMDP & $7.401\times10^4$ & $10$ & $10^5$ & $248$ & $0.5$ & $68.708$ & $302.855$ \\
        (difficult) & UMDP & $5.932\times10^4$ & $10$ & $10^6$ & $285$ & $0.241$ & $61.583$ & $200.311$ \\
        & UMDP & $7.401\times10^4$ & $10$ & $10^6$ & $285$ & $0.165$ & $75.430$ & $207.516$ \\
        & IMDP (Learn Support) & $7.401\times10^4$ & $10$ & $10^6$ & $285$ & $0.166$ & $25.109$ & $21.606$ \\
        & Na\"ive IMDP & $5.932\times10^4$ & $10$ & $10^7$ & $340$ & $0.870$ & $45.865$ & $3.68$ \\
        & UMDP & $5.932\times10^4$ & $10$ & $10^7$ & $353$ & $0.170$ & $70.593$ & $178.599$ \\
        %& UMDP & $7.401\times10^4$ & $10$ & $10^7$ & $345$ & $0.1848$ & $62.510$ & $63.437$ \\
        \midrule
        Multiplicative & UMDP & $3.6\times10^{3}$ & $1$ & $4.705\times10^{3}$  & $247$ & $0.369$ & $0.156$ & $0.051$ \\
        noise ($\varphi_1$) & IMDP (Learn Support) & $3.6\times10^{3}$ & $1$ & $4.371\times10^{3}$  & $247$ & $0.377$ & $0.156$ & $0.011$ \\
        \cite{skovbekk2023formal} & UMDP & $3.6\times10^{3}$ & $1$ & $4.725\times10^{4}$  & $306$ & $0.296$ & $0.194$ & $0.064$ \\
        & UMDP & $3.6\times10^{3}$ & $1$ & $4.722\times10^{5}$  & $312$ & $0.258$ & $0.199$ & $0.070$ \\
        & UMDP & $9.22\times10^{3}$ & $1$ & $4.722\times10^{5}$  & $309$ & $0.243$ & $0.594$ & $0.306$ \\
        & IMDP & $9.22\times10^{3}$ & $1$ & $4.722\times10^{5}$  & $309$ & $0.256$ & $0.594$ & $0.063$ \\
        &\cite{gracia2024data} & $10^{4}$ & $1$ & $4.66\times10^{5}$  & $1066$ & $0.323$ & $13.149$ & $3.863$ \\
        \midrule
        $2D$ Unicycle ($\varphi_2$) & IMDP (Learn Support) & $3.6\times10^3$ & $8$& $5\times10^{3}$ & $36$ & $0.135$  & $0.257$ & $4.527$\\
        \cite{gracia2024data} & UMDP & $3.6\times10^3$ & $8$& $5\times10^{3}$ & $36$ & $0.087$  & $0.257$ & $9.012$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{4}$ & $35$ & $0.038$  & $0.254$ & $7.013$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{5}$ & $41$ & $0.003$  & $0.294$ & $5.622$\\
         %& UMDP & $3.6\times10^3$ & $8$& $10^{6}$ & $43$ & $0.003$  & $0.390$ & $2.767$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{7}$ & $45$ & $0.000$  & $0.321$ & $4.341$\\
         & \cite{gracia2024data} & $3.6\times10^3$ & $8$ & $10^{7}$ & $46$ & $0.030$  & $0.106$ & $3.043$\\
         \midrule
         4-Room Heating ($\varphi_3$) & UMDP & $2.074\times 10^4$ & $16$ & $5\times 10^4$ & $620$ & $0.042$ & $143.869$ & $5.739$\\
         \cite{abate2010approximate} & IMDP (Learn Support) & $2.074\times 10^4$ & $16$ & $5\times 10^4$ & $620$ & $0.102$ & $129.381$ & $2.99$\\
         & UMDP & $2.074\times 10^4$ & $16$ & $5\times 10^5$ & $753$ & $0.020$ & $258.441$ & $6.127$\\
        %& UMDP & $2.074\times 10^4$ & $16$ & $10^6$ & $818$ & $0.044$ & $282.854$ & $7.156$\\
         %& IMDP (Learn Support) & $2.074\times 10^4$ & $16$ & $10^6$ & $818$ & $0.069$ & $204.963$ & $3.296$
    \end{tabular}
    }
    \label{tab:case_studies}
\end{table}

We compare our approach against \citep{gracia2024data}, %the only related work addressing the same problem, 
in Case Studies $1,3,5$-$6$. $2$ is a more challenging version of $1$, where $W$ is bigger and the pendulum cannot swing up in one attempt due to control saturation. Similarly, $4$ extends $3$ with unbounded noise of larger variance and a smaller goal set. Note that \citep{gracia2024data} relies on ambiguity set learning and cannot handle an unbounded $\w$.  We also show results obtained using a na\"ive IMDP abstraction with and without learned support, to show tightness of our approach.
%\ml{add a few case studies to compare new alg. against linprog.}
% In this section, we empirically demonstrate the effectiveness of our approach through seven case studies. These include: 1) a nonlinear pendulum under aerodynamic drag disturbance, 2) kinematic unicycle models with 2- and 3-dimensional state spaces under nonlinear Coulomb friction, 3) a 2-dimensional linear system with multiplicative noise, and 4) a 4-dimensional thermal regulation benchmark modified to account for multiplicative uncertainty. We compare our approach to \cite{gracia2024data}, the only related work addressing the same problem, in Case Studies 1, 3, and 5–6. Case Study 2 presents a more challenging version of Case Study 1, involving unbounded disturbances and control saturation preventing a single swing-up. Similarly, Case Study 4 extends Case Study 3 with unbounded noise of larger variance and a smaller goal set. Notably, \cite{gracia2024data} relies on ambiguity set construction and cannot handle unbounded disturbances.
% We also show results obtained using a na\"ive IMDP abstraction (see Section~\ref{sec:issues}) with and without learned support.
% , i.e., when $\Gamma_{s,a}$ in \eqref{eq:Gamma} is defined by the first and last constraints. 
% The considered specifications are reach-avoid ($\varphi_1$), the \LTLf specification from \cite{gracia2024data} ($\varphi_2$) and a $15$-step safety specification ($\varphi_3$). 
% We present a summary of our results in Table~\ref{tab:case_studies}. These results clearly show the superiority of our approach against \citep{gracia2024data}: the sample complexity is reduced by orders of magnitude, and the size of the abstraction can also be made smaller while yielding similar or tighter results, which also improves the abstraction time in most cases. For abstraction of the same size and, in most cases, the synthesis time is also smaller than the one reported in \citep{gracia2024data}, sometimes by an order of magnitude. Table~\ref{tab:case_studies} also shows that our approach yields tighter results than using na\"ive IMDP, demonstrating the effectiveness of learning additional information in the definition of $\Gamma$ at the cost of a higher computational effort. 
 Table~\ref{tab:case_studies} summarizes our results, highlighting the clear advantages of our approach over \citep{gracia2024data}. Our method significantly reduces sample complexity, often by orders of magnitude, allowing for smaller abstractions while achieving tighter results, thus reducing computation times in most cases. For abstractions of the same size, our synthesis time is typically smaller, sometimes by an order of magnitude. Additionally, the table demonstrates that our approach produces tighter results (less error hence higher probabilistic guarantees) than using a na\"ive IMDP, showcasing the benefits of incorporating additional information into the definition of $\Gamma$, albeit with higher computational effort. Furthermore, UMDPs yield a smaller error, less than a half in some case studies, than when the abstraction is just an IMDP with an additional constraint related to learning the support of $P_W$, showing the benefit of a $2$-layer partition. We also compared the performance of Alg.~\ref{alg:2O} against the linear programming solver \emph{Linprog} on an abstraction with $|S| = 1600$ and $|A| = 8$, achieving the same guarantees but reducing the total synthesis time from 
% $48$ min to $1$ min.
$2880$s to $60$s, a reduction of $48\times$.





%


==> Sections/5_case_studies_old.tex <==
\section{Case Studies}
\label{sec:case_studies}

We now demonstrate empirically the effectiveness of our approach through $7$ case studies. These include a nonlinear pendulum with non-additive %under an aerodynamic drag 
disturbances, kinematic unicycle models with $2$- and $3$-D state-spaces and under nonlinear coulomb friction, a $2$-D linear system with multiplicative noise, and a $4$-D thermal regulation benchmark with multiplicative uncertainty. The considered specifications are reach-avoid ($\varphi_1$), the \LTLf specification from \cite{gracia2024data} ($\varphi_2$) and a $15$-step safety specification ($\varphi_3$). For details of these %systems, specifications, and case study 
setups, see Appendix~\ref{app:appendix_B_arXiv}.

\begin{table}[t]
    \centering
    \caption{\small
    % Benchmark results. In ``Approach'' we indicate what is the abstraction we used: UMDP denotes an abstraction as in Definition~\ref{def:robust_mdp}, ``IMDP (Learn Support)'' refers to a UMDP having only the first and third constraints in \eqref{eq:Gamma}, and ``Na\"ive IMDP'' denotes a traditional IMDP abstraction. $e_{avg}$ denotes the average difference (over all states) between the lower and upper bounds in the satisfaction probabilities. The time required for abstraction and synthesis are given in minutes. %, for which respective timeouts of $8$ and $2$ hours are fixed.
    % We denote the number of samples of the noise after clustering by $N_\text{cluster}$.
    Benchmark results. ``Approach" indicates the abstraction used: UMDP (Definition~\ref{def:robust_mdp}), ``IMDP (Learn Support)" (a UMDP with only the first and third constraints in \eqref{eq:Gamma}), and ``Na\"ive IMDP" (traditional IMDP). $e_{avg}$ represents the average difference in satisfaction probabilities between the lower and upper bounds across all states. Time for abstraction and synthesis is given in minutes, and $ N_\text{cluster}$ denotes the number of noise samples after clustering.
    }
    \scalebox{0.66}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        System (Spec.) & Approach & $|Q|$ & $|A|$ & $N$ & $N_\text{cluster}$ & $e_{avg}$ & Abstr. Time & Synth. Time \\
        \midrule
        Pendulum ($\varphi_1$) & UMDP & $10^4$ & $5$ & $5\times 10^3$ & $47$ & $0.552$ & $1.796$ & $3.643$ \\
        \cite{gracia2024data} & UMDP & $10^4$ & $5$ & $10^4$ & $44$ & $0.007$ & $1.857$ & $6.679$ \\
        & UMDP & $10^4$ & $5$ & $10^5$ & $47$ & $0.003$ & $1.797$ & $2.515$ \\
        %& UMDP & $4\times10^4$ & $5$ & $10^{6}$ & $47$ & $0$ & $7.915$ & $84.539$ \\
        & \cite{gracia2024data} & $4\times10^4$ & $5$ & $10^{6}$ & $49$ & $0$ & $5.273$  & $61.167$ \\
         %&  &  &  & $0.018$ & $-$ & $-$ & $-$ & timeout & $-$ \\
        \midrule
        Pendulum ($\varphi_1$) & UMDP & $1.225\times 10^5$ & $5$ & $5\times10^4$ & $320$ & $0.136$ & $138.705$ & $187.653$ \\
        (Torque-Limited)& UMDP & $6.25\times 10^4$ & $5$ & $10^5$ & $175$ & $0.082$ & $40.602$ & $70.773$ \\
        & UMDP & $4\times 10^4$ & $5$ & $10^5$ & $172$ & $0.279$ & $25.751$ & $42.321$ \\
        & UMDP & $4\times 10^4$ & $5$ & $10^6$ & $179$ & $0.058$ & $26.694$ & $39.667$ \\
        & UMDP & $4\times 10^4$ & $5$ & $10^7$ & $191$ &  $0.033$ & $27.852$ & $27.066$ \\
        & IMDP (Learn Support) & $4\times 10^4$ & $5$ & $10^7$ & $191$ &  $0.172$ & $14.474$ & $20.281$ \\
        \midrule
        $3D$ Unicycle ($\varphi_1$) & UMDP & $5.932\times10^4$ & $10$ & $10^{4}$ & $235$ & $0.579$ & $34.689$ & $33.156$ \\
        \cite{gracia2024data} & UMDP & $5.932\times10^4$ & $10$ & $10^{5}$ & $325$ & $0.267$ & $45.610$ & $36.18$ \\
        & UMDP & $5.932\times10^4$ & $10$ & $10^{6}$ & $358$ & $0.156$ & $52.733$ & $33.751$ \\
        & \cite{gracia2024data} & $6.4\times10^4$ & $10$ & $5\times10^{8}$ & $8869$ & $0.447$ & $457.431$ & $43.342$\\
        \midrule
        $3D$ Unicycle ($\varphi_1$) & UMDP & $7.401\times10^4$ & $10$ & $10^5$ & $269$ & $0.404$ & $48.057$ & $75.164$ \\
        (difficult) & UMDP & $5.932\times10^4$ & $10$ & $10^6$ & $589$ & $0.312$ & $87.753$ & $56.221$ \\
        & UMDP & $7.401\times10^4$ & $10$ & $10^6$ & $295$ & $0.249$ & $53.371$ & $69.565$ \\
        & IMDP (Learn Support) & $7.401\times10^4$ & $10$ & $10^6$ & $295$ & $0.6923$ & $25.109$ & $38.680$ \\
        & Na\"ive IMDP & $5.932\times10^4$ & $10$ & $10^7$ & $340$ & $0.870$ & $45.865$ & $3.68$ \\
        & UMDP & $5.932\times10^4$ & $10$ & $10^7$ & $357$ & $0.199$ & $54.505$ & $47.365$ \\
        & UMDP & $7.401\times10^4$ & $10$ & $10^7$ & $345$ & $0.1848$ & $62.510$ & $63.437$ \\
        \midrule
        Multiplicative & UMDP & $3.6\times10^{3}$ & $1$ & $4.652\times10^{3}$  & $231$ & $0.316$ & $0.294$ & $0.302$ \\
        noise ($\varphi_1$) & IMDP (Learn Support) & $3.6\times10^{3}$ & $1$ & $4.371\times10^{3}$  & $235$ & $0.437$ & $0.412$ & $0.086$ \\
        \cite{skovbekk2023formal} & UMDP & $3.6\times10^{3}$ & $1$ & $4.68\times10^{4}$  & $257$ & $0.251$ & $0.339$ & $0.034$ \\
        & UMDP & $9.6\times10^{3}$ & $1$ & $4.66\times10^{5}$  & $279$ & $0.223$ & $1.150$ & $0.146$ \\
        & IMDP & $9.6\times10^{3}$ & $1$ & $4.66\times10^{5}$  & $276$ & $0.307$ & $0.228$ & $0.034$ \\
        &\cite{gracia2024data} & $10^{4}$ & $1$ & $4.66\times10^{5}$  & $1066$ & $0.323$ & $13.149$ & $3.863$ \\
        \midrule
        $2D$ Unicycle ($\varphi_2$) & UMDP & $3.6\times10^3$ & $8$& $10^{3}$ & $32$ & $0.288$  & $0.302$ & $3.304$\\
         \cite{gracia2024data} & IMDP (Learn Support) & $3.6\times10^3$ & $8$& $5\times10^{3}$ & $31$ & $0.387$  & $0.291$ & $1.174$\\
         & UMDP & $3.6\times10^3$ & $8$& $5\times10^{3}$ & $34$ & $0.095$  & $0.318$ & $2.818$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{4}$ & $37$ & $0.062$  & $0.341$ & $3.103$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{5}$ & $41$ & $0.017$  & $0.375$ & $3.075$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{6}$ & $43$ & $0.003$  & $0.390$ & $2.767$\\
         & UMDP & $3.6\times10^3$ & $8$& $10^{7}$ & $45$ & $0.001$  & $0.408$ & $2.667$\\
         & \cite{gracia2024data} & $3.6\times10^3$ & $8$ & $10^{7}$ & $46$ & $0.03$  & $0.106$ & $3.043$\\
         \midrule
         4-Room Heating ($\varphi_3$) & UMDP & $2.074\times 10^4$ & $16$ & $5\times 10^4$ & $620$ & $0.086$ & $188.506$ & $6.296$\\
         %\cite{abate2010approximate} & UMDP (bigger clusters) & $2.074\times 10^4$ & $16$ & $5\times 10^4$ & $620$ & $0.124$ & $201.496$ & $11.832$\\
         \cite{abate2010approximate} & UMDP & $2.074\times 10^4$ & $16$ & $10^6$ & $818$ & $0.044$ & $282.854$ & $7.156$\\
         & IMDP (Learn Support) & $2.074\times 10^4$ & $16$ & $10^6$ & $818$ & $0.069$ & $204.963$ & $3.296$
    \end{tabular}
    }
    \label{tab:case_studies}
\end{table}

We compare our approach against \cite{gracia2024data}, the only related work addressing the same problem, in Case Studies $1,3,5$-$6$. $2$ is a more challenging version of $1$, where $\w$ is unbounded and the pendulum cannot swing up in one go due to control saturation. Similarly, $4$ extends $3$ with unbounded noise of larger variance and a smaller goal set. Note that \cite{gracia2024data} relies on ambiguity set learning and cannot handle an unbounded $\w$.  We also show results obtained using a na\"ive IMDP abstraction with and without learned support, to show tightness of our approach. Additionally, we show the results of our approach for case studies $\#2$ and $\#6$ in Figure \ref{fig:results}, and for case study $\#4$ in Figure~\ref{fig:IMDP_example}.
%\ml{add a few case studies to compare new alg. against linprog.}
% In this section, we empirically demonstrate the effectiveness of our approach through seven case studies. These include: 1) a nonlinear pendulum under aerodynamic drag disturbance, 2) kinematic unicycle models with 2- and 3-dimensional state spaces under nonlinear Coulomb friction, 3) a 2-dimensional linear system with multiplicative noise, and 4) a 4-dimensional thermal regulation benchmark modified to account for multiplicative uncertainty. We compare our approach to \cite{gracia2024data}, the only related work addressing the same problem, in Case Studies 1, 3, and 5–6. Case Study 2 presents a more challenging version of Case Study 1, involving unbounded disturbances and control saturation preventing a single swing-up. Similarly, Case Study 4 extends Case Study 3 with unbounded noise of larger variance and a smaller goal set. Notably, \cite{gracia2024data} relies on ambiguity set construction and cannot handle unbounded disturbances.
% We also show results obtained using a na\"ive IMDP abstraction (see Section~\ref{sec:issues}) with and without learned support.
% , i.e., when $\Gamma_{s,a}$ in \eqref{eq:Gamma} is defined by the first and last constraints. 
% The considered specifications are reach-avoid ($\varphi_1$), the \LTLf specification from \cite{gracia2024data} ($\varphi_2$) and a $15$-step safety specification ($\varphi_3$). 
% We present a summary of our results in Table~\ref{tab:case_studies}. These results clearly show the superiority of our approach against \cite{gracia2024data}: the sample complexity is reduced by orders of magnitude, and the size of the abstraction can also be made smaller while yielding similar or tighter results, which also improves the abstraction time in most cases. For abstraction of the same size and, in most cases, the synthesis time is also smaller than the one reported in \cite{gracia2024data}, sometimes by an order of magnitude. Table~\ref{tab:case_studies} also shows that our approach yields tighter results than using na\"ive IMDP, demonstrating the effectiveness of learning additional information in the definition of $\Gamma$ at the cost of a higher computational effort. 
 Table~\ref{tab:case_studies} summarizes our results, highlighting the clear advantages of our approach over \cite{gracia2024data}. Our method significantly reduces sample complexity, often by orders of magnitude, and allows for smaller abstractions while achieving similar or tighter results, which also reduces abstraction time in most cases. For abstractions of the same size, our synthesis time is typically smaller, sometimes by an order of magnitude. Additionally, the table demonstrates that our approach produces tighter results (less error hence higher probabilistic guarantees) than using a na\"ive IMDP, showcasing the benefits of incorporating additional information into the definition of $\Gamma$, albeit with higher computational effort. Furthermore, Table~\ref{tab:case_studies} also shows how the probabilistic satisfaction guarantees become tighter with the number of samples, which can also be observed in Figure~\ref{fig:results}, and as the size of the abstraction increases. We also compared the performance of Alg.~\ref{alg:2O} against the linear programming solver \emph{Linprog} on an abstraction with $|S| = 1600$ and $|A| = 8$, achieving the same guarantees but reducing the total synthesis time from 
% $48$ min to $1$ min.
$2880$s to $60$s, a reduction of $48\times$.

%
\begin{figure}[h]
    \begin{minipage}[b]{.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/results_paper_N5_palette2.pdf}
        \subcaption{Pendulum ($N=10^5$)}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.3\linewidth}
    \centering
        \includegraphics[width=\linewidth]{images/results_paper_N6_palette2.pdf}
        \subcaption{Pendulum ($N=10^6$)}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.3\linewidth}
    \centering
        \includegraphics[width=\linewidth]{images/results_paper_N7_palette2.pdf}
        \subcaption{Pendulum ($N=10^7$)}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/unicycle2D_N3_pallette2.pdf}
        \subcaption{$2$D Unicycle ($N=10^3$)}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.3\linewidth}
    \centering
        \includegraphics[width=\linewidth]{images/unicycle2D_N4_pallette2.pdf}
        \subcaption{$2$D Unicycle ($N=10^4$)}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.3\linewidth}
    \centering
        \includegraphics[width=\linewidth]{images/unicycle2D_N6_pallette2.pdf}
        \subcaption{$2$D Unicycle ($N=10^6$)}
    \end{minipage}
    \caption{Synthesis results obtained in case studies $\#3$ (Figures (a-c)) and $\#6$ (Figures (d-f)). The figures show the lower bound in the probability of satisfying $\varphi_1$ and $\varphi_2$, respectively, along with trajectories of the system in closed loop with the synthesized strategy. It can be observed that increasing the number of samples raises this lower bound, and that all trajectories satisfy the respective specification.}
    \label{fig:results}
\end{figure}
%


%


==> Sections/6_conclusion.tex <==
\section{Conclusion}

We propose an approach to synthesize strategies for nonlinear stochastic systems with unknown disturbances via abstractions to UMDPs. We also identify pitfalls in the use of na\"ive abstractions for nonlinear systems and present a synthesis algorithm tailored to our UMDP class. Our extensive case studies show the efficacy and advantages of our framework w.r.t. existing works. In future research we plan to increase the tightness of our results by including additional information into the UMDP and investigate overlapping clusters.

==> Sections/alg.tex <==
\begin{algorithm}[t]\small
\caption{$2$-layer $O$-maximization}\label{alg:2O}
\KwIn{$\M, s \in S, a \in A, \underline{p}^k$}
\KwOut{$\gamma$}
Sort $S$ according to $\{\underline{p}^k(s')\}_{s' \in S}$ in increasing order\;
$\gamma(s') \gets \underline{P}(s, a)(s')$ for all $s' \in \text{Post}(s, a)$\;
$\gamma(s') \gets 0$ for all $s' \notin \text{Post}(s, a)$\;
$\gamma(q') \gets \sum_{s' \in q'} \gamma(s')$ for all $q' \in Q(s, a)$\;
$M \gets 1 - \sum_{s' \in S} \gamma(s')$\;

\For{$q' \in Q(s, a)$}{
    $m \gets \underline{P}(s, a)(q') - \gamma(q')$\;
    \If{$m > 0$}{
        \For{$s' \in q'$}{
            $g \gets \min\{m, \overline{P}(s, a)(s') - \gamma(s')\}$\;
            $\gamma(s') \gets \gamma(s') + g$\;
            $\gamma(q') \gets \gamma(q') + g$\;
            $m \gets m - g$\;
            $M \gets M - g$\;
        }
    }
}

\For{$s' \in \text{Post}(s, a)$}{
    $q' \gets$ get cluster $q'$ such that $s' \in q'$\;
    \eIf{$q' \neq \emptyset$}{
        $m \gets \min\{M, \overline{P}(s, a)(q') - \gamma(q'), \overline{P}(s, a)(s') - \gamma(s')\}$\;
        $\gamma(q') \gets \gamma(q') + m$\;
    }{
        $m \gets \min\{M, \overline{P}(s, a)(s') - \gamma(s')\}$\;
    }
    $\gamma(s') \gets \gamma(s') + m$\;
    $M \gets M - m$\;
}
\end{algorithm}

==> Sections/naiive_imdp.tex <==
\subsection{Issues of Na\"ive Data-Driven IMDP Abstractions}
\label{sec:issues}

\ml{move this section to the supplementary material.}

% As mentioned above, compared to the abstraction classes frequently used in the literature, namely, interval MDPs (IMDPs) \ig{cite}, our UMDP abstraction differs in that the sets $\Gamma_{s,a}$ of transition probability distributions are defined by more constraints than just the intervals $[\underline P(r_s,a)(r_{s'}), \overline P(r_s,a)(r_{s'})]$ for all $s'\in S$. Here, we discuss why IMDPs are not a good abstraction choice in our setting, and thus why a more complex $\Gamma$ is required.

As noted earlier, unlike the commonly used abstraction classes in the literature, such as interval MDPs (IMDPs) \ig{cite}, our UMDP abstraction defines the sets $\Gamma_{s,a}$ of transition probability distributions with more constraints than just the intervals $[\underline P(r_s,a)(r_{s'}), \overline P(r_s,a)(r_{s'})]$ for all $s' \in S$. Below, we explain why IMDPs are unsuitable for our setting and why a more complex definition of $\Gamma$ is necessary through an example.
%
\begin{example}
    Let $\mathcal{I}$ be a UMDP abstraction of System~\eqref{eq:sys}, where $\Gamma$ is only represented by the interval bounds $\underline P(r_s,a)(r_{s'}), \overline P(r_s,a)(r_{s'})$ for all $s'\in S$, making $\mathcal{I}$ an interval MDP (IMDP). For simplicity and without loss of generality, consider the reach-avoid specification $\varphi := \Diamond\rm{goal}\land \Box( \neg\rm{unsafe})$. %Consider also that the state-space discretization was obtained uniformly gridding $X$.
    Note that the event $\text{Reach}(r_s,a,\boldsymbol{\hat w})\subseteq r_{s'}$ present in \eqref{eq:conditions} rarely happens, since it requires that the reachable set is smaller than the region $r_{s'}$. In turn, this event is uncommon in a big portion of the state-space unless the system's dynamics are $1$-step contractive and that the partition is "aligned" with the dynamics. As a consequence, %when $s'$ is not a terminal state, e.g., the goal or unsafe regions, which are typically way bigger than the rest,
    $\underline P(s,a)(s')$ is very often zero. However, the upper bound $\overline P(s,a)(s')$ behaves very differently: by \eqref{eq:conditions}, $\overline P(s,a)(s') \ge \epsilon$ for all $s'\in S$. %Consider the states $\widehat S := \{s'\in S : \exists i\in\{1,\dots, N\}\:\text{s.t.}\: \text{Reach}(r_s,a,\boldsymbol{\hat w}^{(i)})\bigcap r_{s'} \neq \emptyset\}$, i.e., the set of abstract states $s'$ whose corresponding region $r_{s'}$ intersects the reachable set corresponding to some sample of $\w$, and note that typically $|\widehat S| \ll |S|$. 
    
    Consider now the strategy synthesis process for a simple reach-avoid specification, which is carried out via robust dynamic programming. At each iteration, denote by $S_k$ the set of states with zero value function, i.e., the goal states, and note that, typically, $|S_k| \approx |S|$ during the first iterations. Denote by $\widehat S_k\subseteq S$ the set of abstract states $s$ such that $\underline P(s,a)(s') = 0$ for all $s'\in S_k$, and note that, in general, $|\widehat S| \approx |S|$. Now, by construction of $\I$, the adversary $\xi$ is allowed to pick a distribution over $S$ that assigns probability $\epsilon$ of transitioning to every $s'\in \widehat S$, and that, if $S$ is big enough, the total probability of transitioning to these states adds up to $1$. Note that refining the abstraction eventually leads to this condition. As a result, the value function at the iteration $k+1$ is again zero for all $s\in\widehat S$. This phenomenon yields a vacuous satisfaction probability on a big region of the state space.
\end{example}

